Agile Assessment Methods: Current State of the Art

Agility Assessment (AA) comprises tools, assessment techniques, and frameworks that focus on indicating how a company or a team is applying agile techniques and eventually pointing out problems in adopting agile practices at a project-level, organization-level or individual-level. There are many approaches for AA such as agility assessment models, agility checklists, agility surveys, and agility assessment tools. This report presents the state of the art approaches that support agility assessment.

==> 99-bib.tex <==
@article {austin2004,
	author = {Austin, Rob and Devin, Lee},
	title = {Successful innovation through artful process},
	journal = {Leader to Leader},
	volume = {2004},
	number = {32},
	publisher = {Wiley Subscription Services, Inc., A Wiley Company},
	issn = {1531-5355},
	url = {http://dx.doi.org/10.1002/ltl.76},
	doi = {10.1002/ltl.76},
	pages = {48--55},
	year = {2004},
}

@article{basiri2016:chaosengineering, 
	author={A. Basiri and N. Behnam and R. de Rooij and L. Hochstein and L. Kosewski and J. Reynolds and C. Rosenthal}, 
	journal={IEEE Software}, 
	title={Chaos engineering}, 
	year={2016}, 
	volume={33}, 
	number={3}, 
	pages={35-41}, 
	doi={10.1109/MS.2016.60}, 
	ISSN={0740-7459}, 
	month={May},
}

@InProceedings{bendraou2005:UML4SPM,
	author="Bendraou, Reda
		and Gervais, Marie-Pierre
		and Blanc, Xavier",
	editor="Briand, Lionel
		and Williams, Clay",
	title="UML4SPM: a UML2.0-Based metamodel for software process modelling",
	booktitle="Model Driven Engineering Languages and Systems",
	year="2005",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="17--38",
	isbn="978-3-540-32057-9"
}

@article{gandomani2013obstacles,
  title={Obstacles in moving to agile software development methods at a glance},
  author={Gandomani, Taghi Javdani and Zulzalil, Hazura and Ghani, Abdul Azim Abdul and Sultan, Abu Bakar Md and Nafchi, Mina Ziaei},
  journal={Journal of Computer Science},
  volume={9},
  number={5},
  pages={620},
  year={2013},
  publisher={Science Publications}
}

@misc{booch2003,
	title = {The promise, the limits, the beauty of software},
	type = {Talk},
	author = {Grady Booch},
	year = {2007},
	month = {May},
    howpublished = {https://www.youtube.com/watch?v=QWNbK7A\_6KU},
    note = {Accessed: 2018-04-05},
}

@misc{VersionOne2018,
  author = {VersionOne},
  title = {{The 13th annual state of agile report\textsuperscript{TM} 2019}},
  howpublished = {https://stateofagile.com/},
  year = {2019},
  note = {Accessed: 2020-01-15},
}

@misc{VersionOne2009,
  author = {VersionOne},
  title = {{The 4th annual state of agile report\textsuperscript{TM} 2009}},
  howpublished = {https://stateofagile.com/},
  year = {2009},
  note = {Accessed: 2020-09-25},
}


@misc{VersionOne2020,
  author = {VersionOne},
  title = {{The 14th annual state of agile report\textsuperscript{TM} 2020}},
  howpublished = {https://stateofagile.com/},
  year = {2020},
  note = {Accessed: 2020-09-25},
}

@book{brocke2015,
   title =     {Handbook on business process management 1: introduction, methods, and information systems},
   author =    {Jan vom Brocke, Michael Rosemann (eds.)},
   publisher = {Springer-Verlag Berlin Heidelberg},
   isbn =      {978-3-642-45099-0,978-3-642-45100-3},
   year =      {2015},
   series =    {International Handbooks on Information Systems},
   edition =   {2},
}

@inproceedings{brucker2014:improving-ocl,
  title={Panel discussion: proposals for improving OCL},
  author={Achim D. Brucker and Tony Clark and Carolina Dania and Geri Georg and Martin Gogolla and Fr{\'e}d{\'e}ric Jouault and Ernest Teniente and Burkhart Wolff},
  booktitle={OCL@MoDELS},
  year={2014}
}

@article{chou2002,
	author={Shih-Chien Chou},
	journal={Journal of Object- Oriented Programming},
	title={A process modeling language consisting of high level UML diagrams and low level process language},
	year={2002},
	volume={1},
	number={4},
	pages={137-163},
}

@article{dalmaris2007,
	author={Dalmaris, P
		and Tsui, E 
		and Hall, B
		and Smith, B},
	journal={Business Process Management Journal },
	title={A framework for the improvement of knowledge-intensive business processes},
	year={2007},
	volume={13},
	number={2},
	pages={279-305},
	keywords={},
	doi={10.1108/14637150710740509},
	ISSN={1463-7154},
	month={},
}

@inproceedings{dadam2008,
	author="Dadam, Peter
		and Reichert, Manfred
		and Rinderle, Stefanie
		and Jurisch, Martin
		and Acker, Hilmar
		and G{\"o}ser, Kevin
		and Kreher, Ulrich
		and Lauer, Markus",
	editor="Kaschek, Roland
		and Kop, Christian
		and Steinberger, Claudia
		and Fliedl, G{\"u}nther",
	title="Towards truly flexible and adaptive process-aware information systems",
	booktitle="Information Systems and e-Business Technologies",
	year="2008",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="72--83",
	isbn="978-3-540-78942-0"
}

@article{damyanov2015:dsl,
  title={Domain specific languages in practice},
  author={Ivo Damyanov and Mila Sukalinska},
  journal={International Journal of Computer Applications},
  year={2015},
  month={May}
}

@inproceedings{diciccio2012,
	author="Di Ciccio, Claudio and Mecella, Massimo",
	editor="Abramowicz, Witold
		and Kriksciuniene, Dalia
		and Sakalauskas, Virgilijus",
	title="Mining constraints for artful processes",
	booktitle="Business Information Systems",
	year="2012",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="11--23",
	isbn="978-3-642-30359-3"
}

@inproceedings{dinitto2002,
	author={E. Di Nitto and L. Lavazza and M. Schiavoni and E. Tracanella and M. Trombetta},
	booktitle={Proceedings of the 24th International Conference on Software Engineering. ICSE 2002},
	title={Deriving executable process descriptions from UML},
	year={2002},
	volume={},
	number={},
	pages={155-165},
	doi={10.1109/ICSE.2002.1007964},
	ISSN={},
	month={May},
}

@book{browne2009:drools-book,
 author = {Browne, Paul},
 title = {JBoss drools business rules},
 year = {2009},
 isbn = {1847196063, 9781847196064},
 publisher = {Packt Publishing},
} 

@book{duvall2007continuousIntegration,
  title={Continuous integration: improving software quality and reducing risk},
  author={Duvall, P.M. and Matyas, S. and Glover, A.},
  isbn={9780321630148},
  series={Addison-Wesley Signature Series},
  url={https://books.google.com.br/books?id=PV9qfEdv9L0C},
  year={2007},
  publisher={Pearson Education}
}

@book{firesmith2002:opf,
	author={Donald Firesmith and Brian Henderson-Sellers},
	journal={Journal of Object-Oriented Programming},
	title={The OPEN process framework: an introduction},
	year={2002},
	publisher = {Addison-Wesley},
	isbn = {978-0201675108},
}

@article{fowler2005fluent,
  title={{Fluent Interface}},
  author={Fowler, Martin and Evans, Eric},
  journal={URL http://martinfowler.com/bliki/FluentInterface.html (Accessed: 2018-04-05)},
  year={2005}
}

@book{gamma1995,
  title={{Design patterns: elements of reusable object-oriented software}},
  author={Gamma, Erich and Helm, Richard and Johnson, Ralph and  Vlissides, John},
  year={1995},
  publisher={Pearson Education India}
}

@article{gonzalez-perez2005,
	author="Gonzalez-Perez, Cesar
		and McBride, Tom
		and Henderson-Sellers, Brian",
	title="A metamodel for assessable software development methodologies",
	journal="Software Quality Journal",
	year="2005",
	month="Jun",
	day="01",
	volume="13",
	number="2",
	pages="195--214",
	issn="1573-1367",
	doi="10.1007/s11219-005-6217-7",
	url="https://doi.org/10.1007/s11219-005-6217-7"
}

@article{governatori2005,
	author = {Governatori, Guido},
	title = {Representing business contracts in RuleML},
	journal = {International Journal of Cooperative Information Systems},
	volume = {14},
	number = {02n03},
	pages = {181-216},
	year = {2005},
	doi = {10.1142/S0218843005001092},
	URL = {http://www.worldscientific.com/doi/abs/10.1142/S0218843005001092},
}

@inproceedings{halin2017,
	 author = {Halin, Axel and Nuttinck, Alexandre and Acher, Mathieu and Devroey, Xavier and Perrouin, Gilles and Heymans, Patrick},
	 title = {Yo variability! JHipster: a playground for web-apps analyses},
	 booktitle = {Proceedings of the Eleventh International Workshop on Variability Modelling of Software-intensive Systems},
	 series = {VAMOS '17},
	 year = {2017},
	 isbn = {978-1-4503-4811-9},
	 location = {Eindhoven, Netherlands},
	 pages = {44--51},
	 numpages = {8},
	 url = {http://doi.acm.org/10.1145/3023956.3023963},
	 doi = {10.1145/3023956.3023963},
	 acmid = {3023963},
	 publisher = {ACM},
	 address = {New York, NY, USA},
	 keywords = {case study, variability-related analyses, web-apps},
} 

@article{hansson2009ruby,
  title={{Ruby on rails web framework}},
  author={Hansson, David Heinemeier},
  journal={URL http://www.rubyonrails.org (Accessed: 2018-04-05)},
}

@article{hashmi2018,
	year = {2018},
	journal = {Knowledge and Information Systems},
	title = {Are we done with business process compliance: state-of-the-art and challenges ahead},
	author = {Mustafa Hashmi and Guido Governatori and Ho-Pun Lam and Moe Thandar Wynn},
	publisher = {Springer London},
	keywords = {Business processes, Business process compliance, Norms compliance, Normative requirements, Compliance management framework},
	doi = {10.1007/s10115-017-1142-1},
	url = {https://eprints.qut.edu.au/115274/}
}

@article{hendersonsellers2005,
	title = "A comparison of four process metamodels and the creation of a new generic standard",
	journal = "Information and Software Technology",
	volume = "47",
	number = "1",
	pages = "49 - 65",
	year = "2005",
	issn = "0950-5849",
	doi = "https://doi.org/10.1016/j.infsof.2004.06.001",
	author = "B. Henderson-Sellers and C. Gonzalez-Perez",
	keywords = "Metamodel, Software development, Methodology, Standards"
}

@article{hill2006,
	author={C. Hill and R. Yates and C. Jones and S. L. Kogan},
	journal={IBM Systems Journal},
	title={Beyond predictable workflows: enhancing productivity in artful business processes},
	year={2006},
	volume={45},
	number={4},
	pages={663-682},
	keywords={},
	doi={10.1147/sj.454.0663},
	ISSN={0018-8670},
	month={},
}

@book{humble2010continuousDelivery,
  title={Continuous delivery: reliable software releases through build, test, and deployment automation},
  author={Humble, J. and Farley, D.},
  isbn={9780321670229},
  series={Addison-Wesley Signature Series (Fowler)},
  url={https://books.google.com.br/books?id=6ADDuzere-YC},
  year={2010},
  publisher={Pearson Education}
}

@book{fowler1999refactoring,
  title={Refactoring: improving the design of existing code},
  author={Fowler, Martin and Beck, Kent and Brant, John and Opdyke, William and Roberts, Don},
  year={1999},
  publisher={Addison-Wesley Professional}
}

@InProceedings{adali2016evaluation,
	author="Adal{\i}, Onat Ege
	and {\"O}zcan-Top, {\"O}zden and Demir{\"o}rs, Onur",
	editor="Clarke, Paul M. and O'Connor, Rory V. and Rout, Terry and Dorling, Alec",
	title="Evaluation of Agility Assessment Tools: A Multiple Case Study",
	booktitle="Software Process Improvement and Capability Determination",
	year="2016",
	publisher="Springer International Publishing",
	address="Cham",
	pages="135--149",
	isbn="978-3-319-38980-6"
}

@book{hunt1999,
  year = {1999},
  publisher = {{The pragmatic bookshelf}},
  author = {Andrew Hunt and David Thomas},
  title = {{The Pragmatic Programmer}},
}

@book{huttermann2012devops,
  title={Devops for developers},
  author = {Michael H{ü}ttermann},
  isbn={9781430245704},
  series={Expert's voice in Web development},
  url={https://books.google.com.br/books?id=JfUAkB8AA7EC},
  year={2012},
  publisher={Apress}
}

@techreport{ISO24744-2014,
	type = {Standard},
	key = {ISO 24744:2014},
	month = {Nov},
	year = {2014},
	title = {{ISO/IEC 24744:2014 - Software engineering — metamodel for development methodologies (SEMDM)}},
	volume = {2014},
	address = {Geneva, CH},
	institution = {International Organization for Standardization}
}

@article{kammer2000,
	author="Kammer, Peter J.
	and Bolcer, Gregory Alan
	and Taylor, Richard N.
	and Hitomi, Arthur S.
	and Bergman, Mark",
	title="Techniques for supporting dynamic and adaptive workflow",
	journal="Computer Supported Cooperative Work (CSCW)",
	year="2000",
	month="Nov",
	day="01",
	volume="9",
	number="3",
	pages="269--292",
	issn="1573-7551",
	doi="10.1023/A:1008747109146",
	url="https://doi.org/10.1023/A:1008747109146"
}



@book{kruchten2004:rup,
  title={{The rational unified process: an introduction}},
  author={Kruchten, Philippe},
  year={2004},
  publisher={Addison-Wesley Professional}
}

@techreport{kitchenham2007:guidelineSLR,
	added-at = {2010-10-18T14:00:32.000+0200},
	at = {2009-01-27 02:42:01},
	author = {Kitchenham, Barbara and Charters, Stuart},
	id = {3955888},
	institution = {Keele University and Durham University Joint Report},
	interhash = {aed0229656ada843d3e3f24e5e5c9eb9},
	intrahash = {27b256010a48688388374cf83b619b54},
	keywords = {research.cs.softeng research.support},
	number = {EBSE 2007-001},
	priority = {2},
	timestamp = {2010-10-18T14:00:32.000+0200},
	title = {Guidelines for performing Systematic Literature Reviews in Software Engineering},
	year = {2007},
	month = {Jul}
}

@inproceedings{kuhrmann2013,
	 author = {Kuhrmann, Marco and Fern\'{a}ndez, Daniel M{\'e}ndez and Steenweg, Ragna},
	 title = {Systematic software process development: where do we stand today?},
	 booktitle = {Proceedings of the 2013 International Conference on Software and System Process},
	 series = {ICSSP 2013},
	 year = {2013},
	 isbn = {978-1-4503-2062-7},
	 location = {San Francisco, CA, USA},
	 pages = {166--170},
	 numpages = {5},
	 url = {http://doi.acm.org/10.1145/2486046.2486077},
	 doi = {10.1145/2486046.2486077},
	 acmid = {2486077},
	 publisher = {ACM},
	 address = {New York, NY, USA},
	 keywords = {Software process metamodels, literature review, study},
} 


@article{lammel2003,
     author = {L\"{a}mmel, Ralf and Jones, Simon Peyton},
     title = {Scrap your boilerplate: a practical design pattern for generic programming},
     journal = {SIGPLAN Not.},
     issue_date = {March 2003},
     volume = {38},
     number = {3},
     month = jan,
     year = {2003},
     issn = {0362-1340},
     pages = {26--37},
     numpages = {12},
     url = {http://doi.acm.org/10.1145/640136.604179},
     doi = {10.1145/640136.604179},
     acmid = {604179},
     publisher = {ACM},
     address = {New York, NY, USA},
     keywords = {generic programming, rank-2 types, traversal, type cast},
} 

@inproceedings{lindvall2002,
     author = {Lindvall, Mikael and Basili, Victor R. and Boehm, Barry W. and Costa, Patricia and Dangle, Kathleen and Shull, Forrest and Tesoriero, Roseanne and Williams, Laurie A. and Zelkowitz, Marvin V.},
     title = {{Empirical findings in agile methods}},
     booktitle = {Proceedings of the Second XP Universe and First Agile Universe Conference on Extreme Programming and Agile Methods - XP/Agile Universe 2002},
     year = {2002},
     publisher = {Springer-Verlag},
     address = {London, UK, UK},
}


@article{mangan2002,
 author = {Mangan, Peter and Sadiq, Shazia},
 title = {On building workflow models for flexible processes},
 journal = {Aust. Comput. Sci. Commun.},
 issue_date = {January-February 2002},
 volume = {24},
 number = {2},
 month = jan,
 year = {2002},
 pages = {103--109},
 numpages = {7},
 url = {http://dx.doi.org/10.1145/563932.563918},
 doi = {10.1145/563932.563918},
 acmid = {563918},
 publisher = {IEEE Computer Society Press},
 address = {Los Alamitos, CA, USA},
} 

@inproceedings{miller2001,
 author = {Miller, Granville G.},
 title = {{The characteristics of agile software processes}},
 booktitle = {Proceedings of the 39th International Conference and Exhibition on Technology of Object-Oriented Languages and Systems (TOOLS39)},
 series = {TOOLS '01},
 year = {2001},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
} 

@techreport{mcintyre2008,
  title={{Integrated governance, risk and compliance: improve performance and enhance productivity in federal agencies}},
  author={McIntyre, SR},
  year={2008},
  institution={Technical report, PricewaterhouseCoopers}
}

@book{newman2015:Microservices,
  title={Building Microservices: Designing Fine-Grained Systems},
  author={Newman, S.},
  isbn={9781491950333},
  url={https://books.google.com.br/books?id=jjl4BgAAQBAJ},
  year={2015},
  publisher={O'Reilly Media}
}

@article{pai2004,
     author = {M Pai and M McCulloch and JD Gorman and N Pai and W Enanoria and G Kennedy and P Tharyan and JM Colford},
     title = {{Systematic reviews and meta-analyses: an illustrated, step-by-step guide.}},
     journal = {{The Medical Journal of India}},
     year = {2004},
} 

@article{peffers2007,
  author = {Peffers, Ken and Tuunanen, Tuure and Rothenberger, Marcus and Chatterjee, Samir},
  title = {A design science research methodology for information systems research},
  journal = {J. Manage. Inf. Syst.},
  issue_date = {Number 3 / Winter 2007-2008},
  volume = {24},
  number = {3},
  month = dec,
  year = {2007},
  issn = {0742-1222},
  pages = {45--77},
  numpages = {33},
  url = {http://dx.doi.org/10.2753/MIS0742-1222240302},
  doi = {10.2753/MIS0742-1222240302},
  acmid = {1481768},
  publisher = {M. E. Sharpe, Inc.},
  address = {Armonk, NY, USA},
} 

@article{pelaez1999,
	author = {Peláez, Martha and Moreno, Rafael},
	year = {1999},
	month = {01},
	pages = {21-27},
	title = {{Four dimensions of rules and their correspondence to rule-governed behavior: a taxonomy}},
	volume = {8},
	journal = {Behavioral Development Bulletin}
}

@article{ramos-merino2018,
	author="Ramos-Merino, Mateo
		and Santos-Gago, Juan M.
		and {\'A}lvarez-Sabucedo, Luis M.
		and Alonso-Roris, Victor M.
		and Sanz-Valero, Javier",
	title="BPMN-E2: a BPMN extension for an enhanced workflow description",
	journal="Software {\&} Systems Modeling",
	year="2018",
	month="Mar",
	day="02",
	issn="1619-1374",
	doi="10.1007/s10270-018-0669-2",
	url="https://doi.org/10.1007/s10270-018-0669-2"
}

@inproceedings{redding2009,
	author={G. Redding and M. Dumas and A. H. M. ter Hofstede and A. Iordachescu},
	booktitle={2009 IEEE Conference on Commerce and Enterprise Computing},
	title={Modelling flexible processes with business objects},
	year={2009},
	pages={41-48},
	doi={10.1109/CEC.2009.39},
	ISSN={2378-1963},
	month={July},
}

@article{spinellis2012:git,
	author={D. Spinellis},
	journal={IEEE Software},
	title={Git},
	year={2012},
	volume={29},
	number={3},
	pages={100-101},
	doi={10.1109/MS.2012.61},
	ISSN={0740-7459},
	month={May},
}

@inproceedings{utelemaco2017-bpmnr,
  title={BPMN-R: An extension to BPMN to Represent Software Process Rules: doctoral symposium},
  author={Ulisses Telemaco and Toacy Oliveira},
  booktitle={XV Workshop de Teses e Dissertações em Qualidade de Software (WTDQS 2017)},
  year={2017}
}


@techreport {telemaco2017,
  author = {Ulisses Telemaco and Toacy Oliveira and Renata Mesquita and Glaucia Melo and Paulo Alencar},
  title = {A catalog of software development rules for agile methods},
  institution = {Cheriton School of Computer Science - University of Waterloo},
  year = {2017},
  month= {dec}
}

@inproceedings{telemaco2019-1,
	 author = {Ulisses Telemaco and Toacy Oliveira and Paulo Alencar and Don Cowan},
	 title = {A catalog of bad agile smells for agility assessment},
	 booktitle = {Proceedings of the 2019 Ibero-American Conference on Software Engineering},
	 series = {CIbSE 2019},
	 year = {2019},
	 location = {Havana, Cuba},
	 pages="30--43",
} 


@inproceedings{telemaco2019-2,
	 author = {Ulisses Telemaco and Toacy Oliveira and Paulo Alencar and Don Cowan},
	 title = {A metamodel for representing agile software development projects},
	 booktitle = {Proceedings of the 2019 Ibero-American Conference on Software Engineering},
	 series = {CIbSE 2019},
	 year = {2019},
	 location = {Havana, Cuba},
	 pages={30--43},
} 

@article{telemaco2020,
    author={Ulisses Telemaco and Toacy Oliveira and Paulo Alencar and Don Cowan},
    journal={IEEE Access}, 
    title={{A Catalogue of Agile Smells for Agility Assessment}}, 
    year={2020},
    volume={8},
    number={},
    pages={79239-79259},
}

@book{glass2006,
    author = {Glass, Robert L and DeMarco, Tom},
    title = {Software Creativity 2.0},
    year = {2006},
    isbn = {0977213315},
    publisher = {Developer Dot Star Books},
    address = {Atlanta, Georgia}
}

@inproceedings{travassos2008, 
	author={G. H. Travassos and P. S. M. d. Santos and P. G. Mian and A. C. D. Neto and J. Biolchini}, 
	booktitle={13th IEEE International Conference on Engineering of Complex Computer Systems (iceccs 2008)}, 
	title={{An environment to support large scale experimentation in software engineering}}, 
	year={2008}, 
	pages={193-202}, 
	doi={10.1109/ICECCS.2008.30}, 
	month={March},
}


@inproceedings{travassos2016,
  title={A Checklist-Based Inspection Technique for Business Process Models},
  author={de Mello, Rafael Maiani and Motta, Rebeca Campos and Travassos, Guilherme Horta},
  booktitle={International Conference on Business Process Management},
  pages={108--123},
  year={2016},
  organization={Springer}
}


@techreport{ternite2009:VModellXT,
	type = {Standard},
	author = {Ternité, Thomas and Kuhrmann, Marco},
	year = {2009},
	title = {Das V-Modell XT 1.3 Metamodell},
	address = {Germany},
	institution = {Technische Universität Münchenn}
}

@article{xavier1999:PROMENADE,
  author = {Franch, Xavier and M. Rib, Josep},
  year = {1999},
  month = {05},
  pages = {},
  title = {PROMENADE: a modular approach to software process modelling and enaction}
}

@article{vanderaalst2005,
	title = "Case handling: a new paradigm for business process support",
	journal = "Data \& Knowledge Engineering",
	volume = "53",
	number = "2",
	pages = "129 - 162",
	year = "2005",
	issn = "0169-023X",
	doi = "https://doi.org/10.1016/j.datak.2004.07.003",
	url = "http://www.sciencedirect.com/science/article/pii/S0169023X04001296",
	author = "Wil M.P. van der Aalst and Mathias Weske and Dolf Grünbauer",
	keywords = "Case handling, Workflow management systems, Adaptive workflow, Flexibility, Business process management"
}

@article{wagner2005,
 author = {Wagner, Gerd and Damasio, Carlos Viegas and Antoniou, Grigoris},
 title = {{Towards a general web rule language}},
 journal = {Int. J. Web Eng. Technol.},
 issue_date = {December 2005},
 volume = {2},
 number = {2/3},
 month = dec,
 year = {2005},
 issn = {1476-1289},
 pages = {181--206},
 numpages = {26},
 url = {http://dx.doi.org/10.1504/IJWET.2005.008483},
 doi = {10.1504/IJWET.2005.008483},
 acmid = {1358615},
 publisher = {Inderscience Publishers},
 address = {Inderscience Publishers, Geneva, SWITZERLAND},
 keywords = {reaction rules, rule metamodel, semantic web, software agents, web ontologies, web rule markup languages},
}

@article {waller2013:datascience,
	author = {Waller, Matthew A. and Fawcett, Stanley E.},
	title = {Data science, predictive analytics, and big data: a revolution that will transform supply chain design and management},
	journal = {Journal of Business Logistics},
	volume = {34},
	number = {2},
	issn = {2158-1592},
	url = {http://dx.doi.org/10.1111/jbl.12010},
	doi = {10.1111/jbl.12010},
	pages = {77--84},
	year = {2013},
}

@article{karsai2014,
  author    = {Gabor Karsai and
               Holger Krahn and
               Claas Pinkernell and
               Bernhard Rumpe and
               Martin Schindler and
               Steven V{\"{o}}lkel},
  title     = {Design guidelines for domain specific languages},
  journal   = {CoRR},
  volume    = {abs/1409.2378},
  year      = {2014},
  url       = {http://arxiv.org/abs/1409.2378},
  archivePrefix = {arXiv},
  eprint    = {1409.2378},
  timestamp = {Wed, 07 Jun 2017 14:42:32 +0200},
  biburl    = {http://dblp.org/rec/bib/journals/corr/KarsaiKPRSV14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@misc{lee2014,
   author =       {Cynthia Lee},
   title =        {Traditional development practices will fail for mobile apps},
   editor =       {Gartner},
   month =        {August},
   year =         {2014},
   url =          {https://www.gartner.com/newsroom/id/2823619},
   note =         {[Online; posted 14-August-2014]},
 }
 
@article{ly2009,
	title = {On enabling integrated process compliance with semantic constraints in process management systems},
	author = {Linh Thao Ly and Stefanie Rinderle-Ma and Kevin G{\"o}ser and Peter Dadam},
	publisher = {Springer},
	year = {2009},
	pages = {1--25},
	journal = {Information Systems Frontiers},
	url = {http://dbis.eprints.uni-ulm.de/770/},
}

@article{ly2015,
	title = "Compliance monitoring in business processes: functionalities, application, and tool-support",
	journal = "Information Systems",
	volume = "54",
	pages = "209 - 234",
	year = "2015",
	issn = "0306-4379",
	doi = "https://doi.org/10.1016/j.is.2015.02.007",
	url = "http://www.sciencedirect.com/science/article/pii/S0306437915000459",
	author = "Linh Thao Ly and Fabrizio Maria Maggi and Marco Montali and Stefanie Rinderle-Ma and Wil M.P. van der Aalst",
	keywords = "Business process compliance, Compliance monitoring, Operational support"
}

@article{carnaghan2006,
  url = {https://doi.org/10.1016%2Fj.accinf.2005.10.005},
  year = {2006},
  month = {jun},
  publisher = {Elsevier {BV}},
  volume = {7},
  number = {2},
  pages = {170--204},
  author = {Carla Carnaghan},
  title = {{Business process modeling approaches in the context of process level audit risk assessment: an analysis and comparison}},
  journal = {International Journal of Accounting Information Systems},
}

@article{dorling1993,
  author = "A Dorling",
  title = "SPICE: software process improvement and capability determination",
  journal = "Information and Software Technology",
  volume = "35",
  number = "6",
  pages = "404 - 406",
  year = "1993",
  note = "Software Process Modelling in Practice",
  issn = "0950-5849",
  doi = "https://doi.org/10.1016/0950-5849(93)90011-Q",
  url = "http://www.sciencedirect.com/science/article/pii/095058499390011Q",
}

@book{florac1999,
 author = {Florac, William A. and Carleton, Anita D.},
 title = {Measuring the software process: statistical process control for software process improvement},
 year = {1999},
 isbn = {0-201-60444-2},
 publisher = {Addison-Wesley Longman Publishing Co., Inc.},
 address = {Boston, MA, USA},
} 

@incollection{sadiq2011,
  year = {2011},
  publisher = {Springer Nature},
  pages = {1--4},
  author = {Shazia Sadiq},
  title = {{A roadmap for research in business process compliance}},
  booktitle = {Business Information Systems Workshops},
}


@incollection{schultz2014,
  year = {2014},
  publisher = {Springer Nature},
  pages = {184--199},
  author = {Martin Schultz and Michael Radloff},
  title = {{Modeling concepts for internal controls in business processes - an empirically grounded extension of {BPMN}}},
  booktitle = {Lecture Notes in Computer Science},
}


@inproceedings{schultz12,
  author = {Martin Schultz and Niels Mueller-Wickop and Markus Nüttgens},
  year = {2012},
  title = {{Key information requirements for process audits – an expert perspective}},
  booktitle = {Proceedings of the 5th International Workshop on Enterprise Modelling and Information Systems Architectures (EMISA 2012)},
}


@inproceedings{feiler1993,
  publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
  author = {P.H. Feiler and W.S. Humphrey},
  title = {{Software process development and enactment: concepts and definitions}},
  booktitle = {[1993] Proceedings of the Second International Conference on the Software Process-Continuous Software Process Improvement},
  year = {1993},
}


@incollection{sadiq2007,
  publisher = {Springer Nature},
  pages = {149--164},
  author = {Sadiq, Shazia and Governatori, Guido and Namiri, Kioumars},
  title = {{Modeling control objectives for business process compliance}},
  booktitle = {Lecture Notes in Computer Science},
  year = {2007},
}


@incollection{munch2012.2,
  year = {2012},
  publisher = {Springer Nature},
  pages = {139--176},
  author = {Jürgen Münch and Ove Armbrust and Martin Kowalczyk and Mart{\'{\i}}n Soto},
  title = {{Process improvement}},
  booktitle = {The Fraunhofer {IESE} Series on Software and Systems Engineering},
}

@article{bendraou2010,
  year = {2010},
  month = {sep},
  publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
  volume = {36},
  number = {5},
  pages = {662--675},
  author = {Reda Bendraou and Jean-Marc Jezequel and Marie-Pierre Gervais and Xavier Blanc},
  title = {{A comparison of six {UML}-based languages for software process modeling}},
  journal = {{IEEE} Transactions on Software Engineering},
}

@inproceedings{bendraou2007,
  year = {2007},
  month = {aug},
  publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
  author = {Reda Bendraou and Marie-Pierre Gervais},
  title = {{A framework for classifying and comparing process technology domains}},
  booktitle = {International Conference on Software Engineering Advances ({ICSEA} 2007)},
}

@book{weske2012,
  year = {2012},
  publisher = {Springer Nature},
  author = {Mathias Weske},
  title = {{Business Process Management}},
}


@inproceedings{vaculin2011,
  year = {2011},
  month = {aug},
  publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
  author = {Roman Vaculin and Richard Hull and Terry Heath and Craig Cochran and Anil Nigam and Piyawadee Sukaviriya},
  title = {{Declarative business artifact centric modeling of decision and knowledge intensive business processes}},
  booktitle = {2011 {IEEE} 15th International Enterprise Distributed Object Computing Conference},
}


@book{dumas2013,
  year = {2013},
  publisher = {Springer Nature},
  author = {Marlon Dumas and Marcello La Rosa and Jan Mendling and Hajo A. Reijers},
  title = {{Fundamentals of business process management}},
}


@article{garcia2011,
  year = {2011},
  month = {mar},
  publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
  volume = {28},
  number = {2},
  pages = {15--18},
  author = {Felix Garcia and Aurora Vizcaino and Christof Ebert},
  title = {{Process management tools}},
  journal = {{IEEE} Software},
}



@book{munch2012.1,
  year = {2012},
  publisher = {Springer Berlin Heidelberg},
  author = {Jürgen Münch and Ove Armbrust and Martin Kowalczyk and Mart{\'{\i}}n Soto},
  title = {{Software process definition and management}},
}


@article{diciccio2014,
  year = {2014},
  month = {apr},
  publisher = {Springer Nature},
  volume = {4},
  number = {1},
  pages = {29--57},
  author = {Claudio Di Ciccio and Andrea Marrella and Alessandro Russo},
  title = {{Knowledge-intensive processes: characteristics requirements and analysis of contemporary approaches}},
  journal = {Journal on Data Semantics},
}


@article{pillat2015,
  year = {2015},
  month = {jan},
  publisher = {Elsevier {BV}},
  volume = {57},
  pages = {95--115},
  author = {Raquel M. Pillat and Toacy C. Oliveira and Paulo S.C. Alencar and Donald D. Cowan},
  title = {{{BPMNt}: A {BPMN} extension for specifying software process tailoring}},
  journal = {Information and Software Technology},
}


@book{sommerville2010,
  address = {Harlow, England},
  author = {Sommerville, Ian},
  edition = {9},
  isbn = {978-0-13-703515-1},
  publisher = {Addison-Wesley},
  title = {{Software engineering}},
  year = {2010},
}


@inproceedings{fuggetta2000,
  year = {2000},
  publisher = {{ACM} Press},
  author = {Alfonso Fuggetta},
  title = {{Software process}},
  booktitle = {Proceedings of the conference on The future of Software engineering - {ICSE} {\textquotesingle}00},
}

@inproceedings{fuggetta2014,
 author = {Fuggetta, Alfonso and Di Nitto, Elisabetta},
 title = {Software process},
 booktitle = {Proceedings of the on Future of Software Engineering},
 series = {FOSE 2014},
 year = {2014},
 isbn = {978-1-4503-2865-4},
 location = {Hyderabad, India},
 pages = {1--12},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2593882.2593883},
 doi = {10.1145/2593882.2593883},
 acmid = {2593883},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@TechReport{ocl,
  title = {{Object constraint language 2.4 (OCL)}},
  author = {OMG},
  month = {fev},
  year = {2014},
  note = {https://www.omg.org/spec/OCL/2.4/},
  type = {Final Specification},
}

@misc {spring,
    title = {Spring IO},
    author = {Pivotal},
    year = {2016},
    howpublished = {https://spring.io/},
    note = {Accessed: 2018-04-05},
}


@misc {jmock,
    title = {{JMock - an expressive mock object library for java}},
    author = {Steve Freeman and Tim Mackinnon and Nat Pryce and Mauro Talevi and Joe Walnes},
    year = {2016},
    howpublished = {http://jmock.org},
    note = {Accessed: 2018-04-05},
}

@misc {rif:usecases-requirements,
    title = {{RIF use cases and requirements}},
    author = {Allen Ginsberg and David Hirtle and Adrian Paschke and Paula-Lavinia Patranjan and Frank McCabe},
    year = {2008},
    month = {May},
    note = {Accessed: 2018-04-15},
}


@misc {spring-data-jpa,
    title = {Spring data jpa - query methods},
    author = {Pivotal},
    year = {2016},
    howpublished = {https://docs.spring.io/spring-data/jpa/docs/2.1.0.M1/reference/html/#jpa.query-methods},
    note = {Accessed: 2018-04-05},
}

@misc{drools,
  title = {{JBoss drools 7.6.0.final}},
  author = {RedHat},
  year = {2017},
  howpublished = {\url{https://www.drools.org/}},
  note = {Accessed: 2018-04-04},
}

@misc{drl,
  title = {{Drools rule language (DRL)}},
  author = {RedHat},
  year = {2017},
  howpublished = {https://docs.jboss.org/drools/release/7.6.0.Final/drools-docs/html\_single/index.html#\_droolslanguagereferencechapter},
  note = {Accessed: 2018-04-04},
}

@misc{easy-rules,
  title = {{Easy rules 3.1}},
  author = {Mahmoud Ben Hassine},
  year = {2017},
  howpublished = {https://github.com/j-easy/easy-rules},
  note = {Accessed: 2018-04-04},
}

@TechReport{spem,
  title = {{Software Process Engineering Metamodel (SPEM) 2.0 Specification}},
  month = {apr},
  year = {2008},
  note = {http://www.omg.org/spec/SPEM/2.0/PDF/},
  type = {Final Specification},
  institution = {OMG},
  author = {OMG},
}

@book{koenig2007groovy,
  title={Groovy in action},
  author={Koenig, Dierk and Glover, Andrew and King, Paul and Laforge, Guillaume and Skeet, Jon},
  year={2007},
  publisher={Manning Publications Co.}
}

@TechReport{bpmn,
  title = {{Business process model and notation (BPMN)}},
  month = {jan},
  year = {2011},
  note = {http://www.omg.org/spec/BPMN/2.0/},
  type = {Final Specification},
  institution = {OMG},
  author = {OMG},
}



@TechReport{cmmn,
  title = {{Case management model and notation (CMMN)}},
  month = {dez},
  year = {2016},
  note = {http://www.omg.org/spec/CMMN/1.1},
  type = {Final Specification},
  institution = {OMG},
  author = {OMG},
}


@TechReport{dmn,
  title = {{Decison model and notation (DMN)}},
  month = {jun},
  year = {2016},
  note = {http://www.omg.org/spec/DMN/1.1/},
  type = {Final Specification},
  institution = {OMG},
  author = {OMG},
}


@TechReport{spem-2008,
  title = {{Software process engineering metamodel (SPEM) 2.0 specification}},
  month = {apr},
  year = {2008},
  note = {http://www.omg.org/spec/SPEM/2.0/PDF/},
  type = {Final Specification},
  institution = {OMG},
  author = {OMG},
}


@incollection{stroppi2011,
  year = {2011},
  publisher = {Springer Nature},
  pages = {59--73},
  author = {Luis Jes{\'{u}}s Ram{\'{o}}n Stroppi and Omar Chiotti and Pablo David Villarreal},
  title = {{Extending {BPMN} 2.0: method and tool support}},
  booktitle = {Lecture Notes in Business Information Processing},
}


@article{abdullah2016,
  year = {2016},
  month = {feb},
  publisher = {Springer Nature},
  author = {Norris Syed Abdullah and Marta Indulska and Shazia Sadiq},
  title = {{Compliance management ontology - a shared conceptualization for research and practice in compliance management}},
  journal = {Information Systems Frontiers},
}


@article{bierstaker2007,
  year = {2007},
  publisher = {Elsevier {BV}},
  volume = {23},
  pages = {31--48},
  author = {James Bierstaker and Diane Janvrin and D. Jordan Lowe},
  title = {{An examination of factors associated with the type and number of internal control documentation formats}},
  journal = {Advances in Accounting},
}


@inproceedings{schultz2014,
  year = {2014},
  author = {Martin Schultz and Niels Mueller-Wickop},
  title = {{Towards auditors’ preferences on documentation formats in business process audits}},
  booktitle = {Proceedings of the Modellierung 2014},
}


@article{alencar2014,
  year = {2014},
  month = {dec},
  publisher = {American Accounting Association},
  volume = {28},
  number = {2},
  pages = {231--256},
  author = {J. Efrim Boritz and Carla Carnaghan and Paulo S. Alencar},
  title = {{Business modeling to improve auditor risk assessment: an investigation of alternative representations}},
  journal = {Journal of Information Systems},
}


@CONFERENCE{schultz2012,
  author = {Martin Schultz and Niels Mueller-Wickop and Markus Nüttgens},
  title = {{Key information requirements for process audits – an expert perspective}},
  booktitle = {Proceedings of the 5th International Workshop on Enterprise Modelling and Information Systems Architectures (EMISA 2012)},
  year = {2012},
}


@CONFERENCE{wickop2012,
  author = {Niels Mueller-Wickop and Martin Schultz and Markus Nüttgens},
  title = {{Modeling concepts for process audits - an empirically grounded extension of bpmn}},
  booktitle = {Proceedings of the 21st European Conference on Information Systems (ECIS 2013)},
  year = {2013},
}


@inproceedings{dangarska2016,
  year = {2016},
  publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
  author = {Zhivka Dangarska and Kathrin Figl and Jan Mendling},
  title = {{An explorative analysis of the notational characteristics of the decision model and notation ({DMN})}},
  booktitle = {2016 {IEEE} 20th International Enterprise Distributed Object Computing Workshop ({EDOCW})},
}


@incollection{awad2008,
  publisher = {Springer Nature},
  pages = {326--341},
  author = {Ahmed Awad and Gero Decker and Mathias Weske},
  title = {{Efficient compliance checking using {BPMN}-Q and temporal logic}},
  booktitle = {Lecture Notes in Computer Science},
  year = {2008},
}


@incollection{goedertier2006,
  publisher = {Springer Nature},
  pages = {5--14},
  author = {Stijn Goedertier and Jan Vanthienen},
  title = {{Designing compliant business processes with obligations and permissions}},
  booktitle = {Business Process Management Workshops},
}


@incollection{lu2008,
  year = {2008},
  publisher = {Springer Nature},
  pages = {120--131},
  author = {Ruopeng Lu and Shazia Sadiq and Guido Governatori},
  title = {{Compliance aware business process design}},
  booktitle = {Business Process Management Workshops},
}


@incollection{marin2016,
  year = {2016},
  publisher = {Springer International Publishing},
  pages = {5--16},
  author = {Mike A. Marin and Matheus Hauder and Florian Matthes},
  title = {{Case management: an evaluation of existing approaches for knowledge-intensive processes}},
  booktitle = {Business Process Management Workshops},
}


@article{rodriguez2010,
  year = {2010},
  month = {jun},
  publisher = {World Scientific Pub Co Pte Lt},
  volume = {20},
  number = {04},
  pages = {533--548},
  author = {Daniel Rodriguez and Elena Garcia and Salvador Sanches and Carlos Rodriguez-Solano Nuzzi},
  title = {Defining software process model constraints with rules using owl and swrl},
  journal = {International Journal of Software Engineering and Knowledge Engineering},
}

@book{oishi2003,
  year = {2003},
  publisher = {{SAGE} Publications Inc.},
  author = {Sabine Oishi},
  title = {{How to conduct in-person interviews for surveys}},
}


@incollection{schwaber1997,
  year = {1997},
  publisher = {Springer London},
  pages = {117--134},
  author = {Ken Schwaber},
  title = {{{SCRUM} development process}},
  booktitle = {Business Object Design and Implementation},
}


@book{schwaber2002,
  author = {Schwaber, Ken and Beedle, Mike},
  title = {{Agile software development with scrum}},
  year = {2001},
  isbn = {0130676349},
  edition = {1st},
  publisher = {Prentice Hall PTR},
  address = {Upper Saddle River, NJ, USA},
}


@article{beck1999a,
  year = {1999},
  publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
  volume = {32},
  number = {10},
  pages = {70--77},
  author = {K. Beck},
  title = {{Embracing change with extreme programming}},
  journal = {Computer},
}


@book{cockburn2002,
  author = {Cockburn, Alistair},
  title = {{Agile software development}},
  year = {2002},
  isbn = {0-201-69969-9},
  publisher = {Addison-Wesley Longman Publishing Co., Inc.},
  address = {Boston, MA, USA},
}


@book{palmer2001,
  author = {Palmer, Steve R. and Felsing, Mac},
  title = {{A practical guide to feature-driven development}},
  year = {2001},
  isbn = {0130676152},
  edition = {1st},
  publisher = {Pearson Education},
}


@misc{openup,
  author = {Eclipse Foundation},
  title = {{{OpenUp} methodology}},
  year = {2012},
  howpublished = {http://epf.eclipse.org/wikis/openup/},
  note = {Accessed: 2017-12-01},
}


@book{stapleton1997,
  author = {Stapleton, Jennifer},
  title = {{Dynamic systems development method: the method in practice}},
  year = {1997},
  isbn = {0201178893},
  publisher = {Addison-Wesley Longman Publishing Co., Inc.},
  address = {Boston, MA, USA},
}


@book{highsmith2000,
  author = {Highsmith,III, James A.},
  title = {{Adaptive software development: a collaborative approach to managing complex systems}},
  year = {2000},
  isbn = {0-932633-40-4},
  publisher = {Dorset House Publishing Co., Inc.},
  address = {New York, NY, USA},
}


@book{beck1999b,
  author = {Beck, Kent},
  title = {{Extreme programming explained: embrace change}},
  year = {2000},
  isbn = {0-201-61641-6},
  publisher = {Addison-Wesley Longman Publishing Co., Inc.},
  address = {Boston, MA, USA},
}


@misc{fdd,
  author = {Jeff De Luca},
  title = {{Feature driven development {FDD}}},
  howpublished = {http://www.-featuredrivendevelopment.com/},
  year = {1999},
  note = {Accessed: 2017-12-01},
}


@misc{scrum,
  author = {Scrum Alliance},
  title = {{Learn about scrum}},
  howpublished = {https://www.scrumalliance.-org/why-scrum},
  year = {2016},
  note = {Accessed: 2017-12-01},
}


@article{bello2017survey,
  title={A survey on success factors and obstacles for further adoption of agile in IT organisations},
  author={Bello, Mannir and Ghani, Imran},
  journal={International Journal of Advanced Media and Communication},
  volume={7},
  number={3},
  pages={167--180},
  year={2017},
  publisher={Inderscience Publishers (IEL)}
}


@misc{xp,
  author = {Ward Cunningham},
  title = {{Extreme programming}},
  howpublished = {http://www.-extremeprogramming.org/},
  year = {1999},
  note = {Accessed: 2017-12-01},
}

@article{kajornboon2005,
  title={Using interviews as research instruments},
  author={Kajornboon, Annabel Bhamani},
  journal={E-journal for Research Teachers},
  volume={2},
  number={1},
  pages={1--9},
  year={2005}
}

@article{ghazi2017,
  title = {{Survey research in software engineering: problems and strategies}},
  author={Ghazi, Ahmad Nauman and Petersen, Kai and Reddy, Sri Sai Vijay Raj and Nekkanti, Harini},
  journal={arXiv preprint arXiv:1704.01090},
  year={2017}
}


@inproceedings{abrantes2011,
  author = {J. F. Abrantes and G. H. Travassos},
  booktitle = {2011 International Symposium on Empirical Software Engineering and Measurement},
  title = {{Common agile practices in software processes}},
  year = {2011},
  pages = {355-358},
  month = {Sept},
}

@techreport{abrahamsson2002,
  added-at = {2006-06-27T01:17:45.000+0200},
  author = {Abrahamsson, P. and Salo, O. and Ronkainen, J. and Warsta, J.},
  institution = {VTT Publications},
  number = {478},
  title = {{Agile software development methods - review and analysis}},
  year = {2002},
  address = {Espoo, Finland}
}


@misc{beck2001,
  author = {Beck, Kent and Beedle, Mike and van Bennekum, Arie and Cockburn, Alistair and Cunningham, Ward and Fowler, Martin and Grenning, James and Highsmith, Jim and Hunt, Andrew and Jeffries, Ron and Kern, Jon and Marick, Brian and Martin, Robert C. and Mellor, Steve and Schwaber, Ken and Sutherland, Jeff and Thomas, Dave},
  booktitle = {Manifesto for agile software development},
  description = {Manifesto for agile software development},
  title = {{Manifesto for agile software development}},
  howpublished = {http://www.agilemanifesto.org/},
  year = {2001},
}


@misc{berteig2015,
  author = {Mishkin Berteig},
  title = {{Rules of scrum}},
  howpublished = {http://www.agileadvice.com/rules-of-scrum/},
  note = {Accessed: 2017-12-01},
  year = {2015},
}


@article{yu2014,
  title = {{Understanding agile software development practices using shared mental models theory}},
  author = {Xiaodan Yu and Stacie Petter},
  year = {2014},
  volume = {56},
  pages = {911--921},
  journal = {Information and Software Technology},
  publisher = {Elsevier},
  number = {8},
}


@article{dingsoyr2012,
  author = {Dings{\o}yr, Torgeir and Nerur, Sridhar and Balijepally, VenuGopal and Moe, Nils Brede},
  title = {{A decade of agile methodologies}},
  journal = {J. Syst. Softw.},
  issue_date = {June, 2012},
  volume = {85},
  number = {6},
  month = {jun},
  year = {2012},
  pages = {1213--1221},
  numpages = {9},
  publisher = {Elsevier Science Inc.},
  address = {New York, NY, USA},
}


@article{misra2009,
  author = {Misra, Subhas Chandra and Kumar, Vinod and Kumar, Uma},
  title = {{Identifying some important success factors in adopting agile software development practices}},
  journal = {J. Syst. Softw.},
  volume = {82},
  number = {11},
  month = {nov},
  year = {2009},
  pages = {1869--1890},
  numpages = {22},
  publisher = {Elsevier Science Inc.},
  address = {New York, NY, USA},
}


@book{subramaniam2006,
  address = {Raleigh, NC},
  author = {Subramaniam, Venkat and Hunt, Andrew},
  publisher = {Pragmatic Bookshelf},
  title = {{Practices of an agile developer: working in the real world}},
  year = {2006},
}


@inproceedings{ktata2009,
  author = {Ktata, Oualid and L{\'e}vesque, Ghislain},
  title = {{Agile development: issues and avenues requiring a substantial enhancement of the business perspective in large projects}},
  booktitle = {Proceedings of the 2nd Canadian Conference on Computer Science and Software Engineering},
  series = {C3S2E '09},
  year = {2009},
  location = {Montreal, Quebec, Canada},
  pages = {59--66},
  numpages = {8},
  publisher = {ACM},
  address = {New York, NY, USA},
}


@book{martin2003,
  author = {Martin, Robert Cecil},
  title = {{Agile software development: principles, patterns, and practices}},
  year = {2003},
  isbn = {0135974445},
  publisher = {Prentice Hall PTR},
  address = {Upper Saddle River, NJ, USA},
}


@inproceedings{chen2011,
  author = {N. Chen and S. C. H. Hoi and X. Xiao},
  booktitle = {2011 26th IEEE/ACM International Conference on Automated Software Engineering (ASE 2011)},
  title = {{Software process evaluation: A machine learning approach}},
  year = {2011},
  pages = {333-342},
  month = {Nov},
}


@inproceedings{he2009,
  author = {X. He and J. Guo and Y. Wang and Y. Guo},
  booktitle = {2009 16th Asia-Pacific Software Engineering Conference},
  title = {{An automatic compliance checking approach for software processes}},
  year = {2009},
  pages = {467-474},
  month = {Dec},
}

@inproceedings{newkirk2002, 
	author={J. Newkirk}, 
	booktitle={Proceedings of the 24th International Conference on Software Engineering. ICSE 2002}, 
	title={Introduction to agile processes and extreme programming}, 
	year={2002}, 
	pages={695-696}, 
	month={May},
}

@inproceedings{simmons2003open,
  title={Open source development and agile methods},
  author={Simmons, G and Dillon, TS},
  booktitle={The 7th International Conference on Software Engineering and Applications},
  year={2003}
}

@article{joseph2005software,
  title={Software engineering: agile manifesto},
  author={Joseph, Meera},
  journal={Elektron Journal-South African Institute of Electrical Engineers},
  volume={22},
  number={9},
  pages={70},
  year={2005},
  publisher={Elektron Management Partnership}
}

@article{cao2007agile,
  title={{Agile software development: ad hoc practices or sound principles?}},
  author={Cao, Lan and Ramesh, Balasubramaniam},
  journal={IT professional},
  volume={9},
  number={2},
  year={2007},
  pages = {41--47},
  publisher={IEEE}
}


@inproceedings{thomas2008,
  title={Introducing agile development practices from the middle},
  author={Thomas, Jann},
  booktitle={Engineering of Computer Based Systems, 2008. ECBS 2008. 15th Annual IEEE International Conference and Workshop on the},
  pages={401--407},
  year={2008},
  organization={IEEE}
}

@inproceedings{kautz2009cultures,
  title={Cultures of agility - agile software development in practice},
  author={Kautz, Karlheinz and Pedersen, Casper Fabricius and Monrad, Ole},
  booktitle={20th Australasian Conference on Information Systems. Melbourne},
  year={2009}
}

@article{mnkandla2009agile,
  title={Agile software engineering},
  author={Mnkandla, Ernest},
  journal={Handbook of Research on Software Engineering and Productivity Technologies: Implications of Globalization: Implications of Globalization},
  pages={28},
  year={2009},
  publisher={IGI Global}
}

@incollection{williams2010agile,
  title={Agile software development methodologies and practices},
  author={Williams, Laurie},
  booktitle={Advances in Computers},
  volume={80},
  pages={1--44},
  year={2010},
  publisher={Elsevier}
}

@book{dingsoyr2010agile,
   author={Dings{\o}yr, Torgeir and Dyb{\aa}, Tore and Moe, Nils Brede},
   year = {2010},
   month = {01},
   title = {Agile software development},
   isbn = {978-3-642-12575-1},
   journal = {Agile Software Development: Current Research and Future Directions, ISBN 978-3-642-12574-4. Springer-Verlag Berlin Heidelberg, 2010},
}



@article{rao2011study,
  title={A study of the agile software development methods, applicability and implications in industry},
  author={Rao, Kuda Nageswara and Naidu, G Kavita and Chakka, Praneeth},
  journal={International Journal of Software Engineering and its applications},
  volume={5},
  number={2},
  pages={35--45},
  year={2011}
}

@incollection{alzoabi2012agile,
  title={Agile software: body of knowledge},
  author={Alzoabi, Zaidoun},
  booktitle={Business Intelligence and Agile Methodologies for Knowledge-Based Organizations: Cross-Disciplinary Applications},
  pages={14--34},
  year={2012},
  publisher={IGI Global}
}

@inproceedings{hamed2013popular,
  title={Popular agile approaches in software development: review and analysis},
  author={Hamed, Amani Mahdi Mohammed and Abushama, Hisham},
  booktitle={Computing, Electrical and Electronics Engineering (ICCEEE), 2013 International Conference on},
  pages={160--166},
  year={2013},
  organization={IEEE}
}

@inproceedings{diebold2014agile,
  title={Agile practices in practice: a mapping study},
  author={Diebold, Philipp and Dahlem, Marc},
  booktitle={Proceedings of the 18th International Conference on Evaluation and Assessment in Software Engineering},
  pages={30},
  year={2014},
  organization={ACM}
}

@incollection{moran2014agile,
  title={Agile software development},
  author={Moran, Alan},
  booktitle={Agile Risk Management},
  pages={1--16},
  year={2014},
  publisher={Springer International Publishing},
  address="Cham"
}

@InProceedings{chagas2014systematic,
	author="Chagas, Larissa Fernandes and de Carvalho, Daniel Dias and Lima, Adailton Magalh{\~a}es an Reis, Carla Alessandra Lima",
	editor="Mitasiunas, Antanas and Rout, Terry and O'Connor, Rory V. and Dorling, Alec",
	title="Systematic Literature Review on the Characteristics of Agile Project Management in the Context of Maturity Models",
	booktitle="Software Process Improvement and Capability Determination",
	year="2014",
	publisher="Springer International Publishing",
	address="Cham",
	pages="177--189",
	isbn="978-3-319-13036-1"
}

@article{anand2016popular,
  title={Popular agile methods in software development: review and analysis},
  author={Anand, R Vijay and Dinakaran, M},
  journal={International Journal of Applied Engineering Research},
  volume={11},
  number={5},
  pages={3433--3437},
  year={2016}
}

@inproceedings{soundararajan2011structured,
  title={A structured framework for assessing the ``goodness'' of agile methods},
  author={Soundararajan, Shvetha and Arthur, James D},
  booktitle={2011 18th IEEE International Conference and Workshops on Engineering of Computer-Based Systems},
  pages={14--23},
  year={2011},
  organization={IEEE}
}

@MISC {yatzeck2012,
    author       = "Elena Yatzeck",
    title        = "A corporate agile 10-point checklist",
    howpublished = "http://pagilista.blogspot.com/2012/12/a-corporate-agile-10-point-checklist.html",
    month        = "Dec",
    year         = "2012",
    note         = "Accessed: 2019-06-30"
}

@book{shore2007art,
  title={{The art of agile development: pragmatic guide to agile software development}},
  author={James Shore and Shane Warden},
  year={2007},
  publisher={" O'Reilly Media, Inc."}
}

@incollection{leppanen2013comparative,
  title={{A comparative analysis of agile maturity models}},
  author={Lepp{\"a}nen, Mauri},
  booktitle={Information Systems Development},
  pages={329--343},
  year={2013},
  publisher={Springer}
}

@misc{larsen2018,
  title = {{The agile fluency model: a brief guide to success with agile}},
  author = {Diana Larsen and James Shore},
  year = {2018},
  howpublished = {https://martinfowler.com/articles/agileFluency.html},
  note = {Accessed: 2019-06-30}
}

@misc{xxxxkrebs2011agile,
  title="Agile journey index",
  author="Krebs, W and Morgan, P and Ashton, R",
  year="2011",
  organization="AgileBill Krebs",
  howpublished = "http://www.agiledimensions.com/blog/wp-content/uploads/2011/10/KrebsAgileJourneyIndex.pdf",
  note = "Accessed: 2019-06-30"
}

@misc{maciver2010,
    title = "Agility maturity self assessment",
    author = "Bryan Campbell and Robbie MacIver",
    year = "2010",
    howpublished = "http://www.robbiemaciver.com/documents/presentations/A2010-Agile\%20Maturity\%20Self-Assessment.pdf",
    note = "Accessed: 2019-06-30"
}

@misc{ribeiro2015,
  title = {{Agility maturity self assessment survey}},
  author = {Eduardo Ribeiro},
  year = {2015},
  howpublished = {https://beyondleanagile.com/2015/12/08/agile-maturity-self-assessment-survey-published-at-scrumalliance/},
  note = {Accessed: 2019-06-30}
}

@misc{xxxxxtousignant2013,
  title = {{How agile are you? free agile maturity assessment}},
  author = {Daniel Tousignant},
  year = {2013},
  howpublished = {https://capeprojectmanagement.com/agile-self-assessment/},
  note = {Accessed: 2019-06-30}
}

@manual{tousignant2019-AgileMaturityMatrix,
    title = {Agile Maturity Matrix},
    author = {Daniel Tousignant},
    year = {2019},
    url = {https://capeprojectmanagement.com/agile-self-assessment/}
}

@manual{tousignant2019-AgileMaturityAssessment,
    title = {Agile Maturity Assessment},
    author = {Daniel Tousignant},
    year = {2019},
    url = {https://capeprojectmanagement.com/individual-assessment/}
}


@manual{waters2008,
  title = {{How agile are you? ((Take This 42 Point Test))}},
  author = {Kelly Waters},
  year = {2008},
  url = {https://www.101ways.com/2008/01/21/how-agile-are-you-take-this-42-point-test/},
  note = {Accessed: 2020-11-01}
}

@misc{ibmDevOpsPracticesSelfAssessment,
  title = {{IBM devops self-assessment}},
  author = {IBM},
  howpublished = {https://devopsassessment.mybluemix.net/},
  note = {Accessed: 2019-06-30},
  year = {2008}
}

@misc{xxxxinfotech2013,
  title = {{Agile process assessment tool}},
  author = {Info Tech Research Group},
  year = {2013},
  howpublished = {https://www.infotech.com/research/ss/it-deploy-changes-more-rapidly-by-going-agile/it-agile-process-assessment-tool},
  note = {Accessed: 2019-06-30}
}

@article{matalonga2015agis,
  title={AGIS: towards an ISO9001 based tool for measuring agility},
  author={Matalonga Motta, Santiago and Rivedieu, Gast{\'o}n},
  journal={Computaci{\'o}n y Sistemas},
  volume={19},
  number={1},
  pages={163--175},
  year={2015}
}

@manual {schumacher2009-borland,
    title = {Borland Agile Assessment 2009},
    author = {Dale Schumacher},
    year = {2009},
    url = {https://borland.typepad.com/agile_transformation/2009/03/borland-agile-assessment-2009.html}
}

@misc{sahotaxxxxxxx,
    author = "Michael Sahota",
    title = "An agile adoption and transformation survival guide",
    howpublished = "http://www.barryovereem.com/wp-content/uploads/M.-Sahota-Checklist-for-Change-Agents.pdf",
    note = "Accessed: 2019-06-30",
    year = "2010"
}

@book{sahota2012-agile-adoption,
  title={An Agile Adoption and Transformation Survival Guide},
  author={Sahota, Michael},
  year={2012},
  publisher={Lulu. com}
}

@inproceedings{williams2010ca,
  title={Driving process improvement via comparative agility assessment},
  author={Williams, Laurie and Rubin, Kenny and Cohn, Mike},
  booktitle={2010 Agile Conference},
  pages={3--10},
  year={2010},
  organization={IEEE}
}

@misc{xxxxxeliassen2013AgilityMatrix,
    author = "Dave MacKeen",
    title = "Enterprise and team level agility maturity matrix",
    howpublished = "http://blog.eliassen.com/introducing-the-enterprise-agility-maturity-matrix",
    year = "2013",
    organization = "Eliassen Group",
    note = "Accessed: 2019-06-30"
}

@misc{kniberg2012scrumchecklist,
    author = "Henrik Kniberg",
    title = "Scrum checklist",
    howpublished = "http://www.crisp.se/scrum/checklist",
    year = "2012",
    note = "Accessed: 2019-06-30"
}

@manual{rothman2013,
  author = "Johanna Rothman",
  title = "Self assessment tool for transitioning to agile",
  url = "https://www.jrothman.com/mpd/agile/2013/04/self-assessment-tool-for-transitioning-to-agile/",
  year = "2013",
  note = "Accessed: 2019-06-30"
}

@InProceedings{fraser2006agile,
	author="Fraser, Steven and Boehm, Barry and J{\"a}rkvik, Jack and Lundh, Erik and Vilkki, Kati",
	editor="Abrahamsson, Pekka and Marchesi, Michele and Succi, Giancarlo",
	title="How Do Agile/XP Development Methods Affect Companies?",
	booktitle="Extreme Programming and Agile Processes in Software Engineering",
	year="2006",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="225--228",
	isbn="978-3-540-35095-8"
}

@article{gandomani2013important,
  title={Important considerations for agile software development methods governance.},
  author={Gandomani, Taghi Javdani and Zulzalil, Hazura and Ghani, Abdul and Azim, Abdul and Sultan, Abu Bakar},
  journal={Journal of Theoretical \& Applied Information Technology},
  volume={55},
  number={3},
  year={2013},
  pages="345--351",
}

@book{ambler2012disciplined,
  title={Disciplined agile delivery: a practitioner's guide to agile software delivery in the enterprise},
  author={Ambler, Scott W and Lines, Mark},
  year={2012},
  publisher={IBM press}
}

@misc{ambler2018survey,
  author = {Scott Ambler},
  title = {{IT project success rates survey results}},
  howpublished={http://www.ambysoft.com/surveys/success2018.html},
  year = {2018},
  note = {Accessed: 2019-10-01},
}


%reference ozcan2015agilitymod updated...
@InProceedings{ozcan-top2015-agilitymod,
	author="Ozcan-Top, Ozden and Demir{\"o}rs, Onur",
	editor="Rout, Terry and O'Connor, Rory V. and Dorling, Alec",
	title="A Reference Model for Software Agility Assessment: AgilityMod",
	booktitle="Software Process Improvement and Capability Determination",
	year="2015",
	publisher="Springer International Publishing",
	address="Cham",
	pages="145--158",
	isbn="978-3-319-19860-6"
}


@article{moha2009decor,
  title={Decor: a method for the specification and detection of code and design smells},
  author={Moha, Naouel and Gueheneuc, Yann-Gael and Duchien, Laurence and Le Meur, Anne-Francoise},
  journal={IEEE Transactions on Software Engineering},
  volume={36},
  number={1},
  pages={20--36},
  year={2009},
  publisher={IEEE}
}


@book{brown1998antipatterns,
  title={AntiPatterns: refactoring software, architectures, and projects in crisis},
  author={Brown, William H and Malveau, Raphael C and McCormick, Hays W and Mowbray, Thomas J},
  year={1998},
  publisher={John Wiley \& Sons, Inc.}
}

@book{lanza2007object,
	title={Object-oriented metrics in practice: using software metrics to characterize, evaluate, and improve the design of object-oriented systems},
	author={Lanza, Michele and Marinescu, Radu},
	year={2007},
	publisher={Springer-Verlag},
	address="Berlin, Heidelberg",
	isbn="978-3-540-24429-5"
}

@inproceedings{van2002java,
  title={Java quality assurance by detecting code smells},
  author={Van Emden, Eva and Moonen, Leon},
  booktitle={Ninth Working Conference on Reverse Engineering, 2002. Proceedings.},
  pages={97--106},
  year={2002},
  organization={IEEE}
}

@inproceedings{travassos1999detecting,
  title={Detecting defects in object-oriented designs: using reading techniques to increase software quality},
  author={Travassos, Guilherme and Shull, Forrest and Fredericks, Michael and Basili, Victor R},
  booktitle={ACM Sigplan Notices},
  volume={34},
  number={10},
  pages={47--56},
  year={1999},
  organization={ACM}
}

@misc{hermida2009abetterteam,
  title = {{A better team}},
  author = {Sebastian Hermida},
  howpublished = {http://www.abetterteam.org/},
  year = {2009},
  note = {Accessed: 2019-06-30}
}


@INPROCEEDINGS{rehman2018, 
    author={F. u. {Rehman} and B. {Maqbool} and M. Q. {Riaz} and U. {Qamar} and M. {Abbas}}, 
    booktitle={2018 21st Saudi Computer Society National Computer Conference (NCC)}, 
    title={Scrum software maintenance model: efficient software maintenance in agile methodology}, 
    year={2018},
    pages={1-5}, 
    doi={10.1109/NCG.2018.8593152}, 
    month={April},
}

@article{tripp2016,
    author = {Tripp, John and Armstrong, Deb},
    year = {2016},
    month = {10},
    pages = {1-10},
    title = {Agile methodologies: organizational adoption motives, tailoring, and performance},
    volume = {58},
    journal = {Journal of Computer Information Systems},
    doi = {10.1080/08874417.2016.1220240}
}


@inproceedings{spinola2008,
    author = {Rodrigo O Spínola and Arilo C Dias-Neto and Guilherme H Travassos},
    year = {2008},
    title = {Abordagem para desenvolver tecnologia de software com apoio de estudos secundários e primários},
    booktitle = {Experimental Software Engineering Latin American Workshop (ESELAW)}
}

@article{fontana2012automatic,
  title={Automatic detection of bad smells in code: An experimental assessment.},
  author={Fontana, Francesca Arcelli and Braione, Pietro and Zanoni, Marco},
  journal={Journal of Object Technology},
  volume={11},
  number={2},
  pages={5--1},
  year={2012}
}

@inproceedings{schumacher2010building,
  title={Building empirical support for automated code smell detection},
  author={Schumacher, Jan and Zazworka, Nico and Shull, Forrest and Seaman, Carolyn and Shaw, Michele},
  booktitle={Proceedings of the 2010 ACM-IEEE International Symposium on Empirical Software Engineering and Measurement},
  pages={8},
  year={2010},
  organization={ACM}
}



@mastersthesis{chronis2015MasterMeasuringAgility,
  title = {Measuring agility - a validity study on tools measuring the agility level of software development teams},
  author = {Chronis, Konstantinos},
  school = {University of Gotherburg},
  address = {Goteborg, Sweden},
  year = {2015}
}

@InProceedings{baloni2016,
	author="Nebe, Karsten and Baloni, Snigdha",
	editor="Yamamoto, Sakae",
	title="Agile Human-Centred Design: A Conformance Checklist",
	booktitle="Human Interface and the Management of Information: Information, Design and Interaction",
	year="2016",
	publisher="Springer International Publishing",
	address="Cham",
	pages="442--453",
	isbn="978-3-319-40349-6"
}

@inproceedings{qumer2006-4DAT,
  title = {Measuring agility and adaptibility of agile methods: A 4 dimensional analytical tool},
  author={Qumer, Asif and Henderson-Sellers, Brian},
  booktitle = {The IADIS international conference on applied computing 2006},
  year = {2006},
  organization = {IADIS Press}
}

@article{qumer2008-agile-adoption,
  title={A framework to support the evaluation, adoption and improvement of agile methods in practice},
  author={Qumer, Asif and Henderson-Sellers, Brian},
  journal={Journal of Systems and Software},
  volume={81},
  number={11},
  pages={1899--1919},
  year={2008},
  publisher={Elsevier}
}

@InProceedings{yurum2018,
	author="Y{\"u}r{\"u}m, Ozan Ra{\c{s}}it and Demir{\"o}rs, Onur and Rabhi, Fethi",
	editor="Stamelos, Ioannis and O'Connor, Rory V. and Rout, Terry and Dorling, Alec",
	title="A Comprehensive Evaluation of Agile Maturity Self-assessment Surveys",
	booktitle="Software Process Improvement and Capability Determination",
	year="2018",
	publisher="Springer International Publishing",
	address="Cham",
	pages="300--315",
	isbn="978-3-030-00623-5"
}

@phdthesis{soundararajan2013-ops,
  title={Assessing agile methods: investigating adequacy, capability, and effectiveness (an objectives, principles, strategies approach)},
  author={Soundararajan, Shvetha},
  year={2013},
  school={Virginia Tech}
}

@InProceedings{so2009-pam,
	author="So, Chaehan and Scholl, Wolfgang", 
	editor="Abrahamsson, Pekka and Marchesi, Michele and Maurer, Frank",
	title="Perceptive Agile Measurement: New Instruments for Quantitative Studies in the Pursuit of the Social-Psychological Effect of Agile Practices",
	booktitle="Agile Processes in Software Engineering and Extreme Programming",
	year="2009",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="83--93",
	isbn="978-3-642-01853-4"
}

@book{leffingwell2007-taa,
  title={Scaling software agility: best practices for large enterprises},
  author={Leffingwell, Dean},
  year={2007},
  publisher={Pearson Education}
}

@book{leffingwell2016-safe,
    author = {Leffingwell, Dean},
    title = {{SAFe 4.0 Reference Guide: Scaled Agile Framework for Lean Software and Systems Engineering}},
    year = {2016},
    isbn = {0134510542},
    publisher = {Addison-Wesley Professional},
    edition = {1st},
}



@inproceedings{gill2006measuring,
  title={Measuring agility and adaptibility of agile methods: a 4 dimensional analytical tool},
  author={Gill, AQ and Henderson-Sellers, Brian},
  booktitle={The IADIS international conference on applied computing 2006},
  year={2006},
  organization={IADIS Press}
}

@article{tsourveloudis2002measurement,
  title={On the measurement of enterprise agility},
  author={Tsourveloudis, Nikos C and Valavanis, Kimon P},
  journal={Journal of Intelligent and Robotic Systems},
  volume={33},
  number={3},
  pages={329--342},
  year={2002},
  publisher={Springer}
}

@article{li2010citation,
  title={Citation analysis: comparison of Web of Science{\textregistered}, Scopus{\textregistered}, SciFinder{\textregistered}, and Google Scholar},
  author={Li, Jie and Burnham, Judy F and Lemley, Trey and Britton, Robert M},
  journal={Journal of electronic resources in medical libraries},
  volume={7},
  number={3},
  pages={196--217},
  year={2010},
  publisher={Taylor \& Francis}
}

%XP primary stidy reference
@article{lindstrom2004extreme,
  title={Extreme programming and agile software development methodologies},
  author={Lindstrom, Lowell and Jeffries, Ron},
  journal={Information systems management},
  volume={21},
  number={3},
  pages={41--52},
  year={2004},
  publisher={Taylor \& Francis}
}

@article{cohen1999pomp,
  title={The problem of units and the circumstance for POMP},
  author={Cohen, Patricia and Cohen, Jacob and Aiken, Leona S and West, Stephen G},
  journal={Multivariate behavioral research},
  volume={34},
  number={3},
  pages={315--346},
  year={1999},
  publisher={Taylor \& Francis}
}

@article{maurer2002,
	title = {Extreme programming: {rapid} development for web-based applications},
	volume = {6},
	number = {1},
	journal = {IEEE Internet Computing},
	author = {Maurer, F. and Martel, S.},
	year = {2002},
	pages = {86--90}
}

@inproceedings{newkirk2002,
	title = {Introduction to agile processes and extreme programming},
	booktitle = {Proceedings - {International} {Conference} on {Software} {Engineering}},
	author = {Newkirk, J.},
	year = {2002},
	
	pages = {695--696}
}

@inproceedings{simmons2003,
	title = {Open source development and {agile} methods},
	volume = {7},
	booktitle = {Proceedings of the {IASTED} {International} {Conference} on {Software} {Engineering} and {Applications}},
	author = {Simmons, G.L. and Dillon, T.},
	year = {2003},
	pages = {523--527}
}

@inproceedings{nisar2004,
	title = {Agile methods handling offshore software development issues},
	doi = {10.1109/INMIC.2004.1492915},
	booktitle = {Proceedings of {INMIC} 2004 - 8th {International} {Multitopic} {Conference}},
	author = {Nisar, M.F. and Hameed, T.},
	year = {2004},
	pages = {417--422}
}

@article{miller2005,
	title = {Agile software development for the entire project},
	volume = {18},
	number = {12},
	journal = {CrossTalk},
	author = {Miller, G.},
	year = {2005},
	pages = {9--12}
}

@InProceedings{pikkarainen2005,
	author="Pikkarainen, Minna and Salo, Outi and Still, Jari",
	editor="Richardson, Ita and Abrahamsson, Pekka and Messnarz, Richard",
	title="Deploying Agile Practices in Organizations: A Case Study",
	booktitle="Software Process Improvement",
	year="2005",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="16--27",
	isbn="978-3-540-32271-9"
}

@article{mcmahon2005,
	title = {Extending agile methods: a distributed project and organizational improvement perspective},
	number = {5},
	journal = {CrossTalk},
	author = {McMahon, P.E.},
	year = {2005},
	pages = {16--19}
}

@inproceedings{elssamadisy2006,
	title = {Adopting agile practices: an incipient pattern language},
	booktitle = {{PLoP} 2006 - {PLoP} {Pattern} {Languages} of {Programs} 2006 {Conference} {Proceedings}},
	author = {Elssamadisy, A. and West, D.},
	year = {2006},
	keywords = {uli-ok}
}

@article{ambler2006,
	title = {Survey says: agile works in practice},
	volume = {31},
	number = {9},
	journal = {Dr. Dobb's Journal},
	author = {Ambler, S.W.},
	year = {2006},
	pages = {62--64}
}

@inproceedings{thomas2008,
	title = {Introducing agile development practices from the middle},
	booktitle = {Proceedings - {Fifteenth} {IEEE} {International} {Conference} and {Workshops} on the {Engineering} of {Computer}-{Based} {Systems}, {ECBS} 2008},
	author = {Thomas, J.},
	year = {2008},
	pages = {401--407}
}

@inproceedings{kautz2009,
	title = {Cultures of agility - agile software development in practice},
	booktitle = {{ACIS} 2009 {Procedings} - 20th {Australasian} {Conference} on {Information} {Systems}},
	author = {Kautz, K. and Pedersen, C.F. and Monrad, O.},
	year = {2009},
	pages = {174--184}
}

@article{batra2009,
	title = {Modified agile practices for outsourced software projects},
	volume = {52},
	number = {9},
	journal = {Communications of the ACM},
	author = {Batra, D.},
	year = {2009},
	pages = {143--148+10}
}

@inproceedings{li2010,
	title = {Research and practice of agile unified process},
	volume = {2},
	booktitle = {{ICSTE} 2010 - 2010 2nd {International} {Conference} on {Software} {Technology} and {Engineering}, {Proceedings}},
	author = {Li, J.},
	year = {2010},
	pages = {V2340--V2343}
}

@article{zhang2010,
	title = {Software development methodologies, trends and implications: a testing centric view},
	volume = {9},
	number = {8},
	journal = {Information Technology Journal},
	author = {Zhang, X. and Hu, T. and Dai, H. and Li, X.},
	year = {2010},
	pages = {1747--1753}
}

@inproceedings{shi2011,
	title = {Agile planning and development methods},
	volume = {1},
	booktitle = {{ICCRD2011} - 2011 3rd {International} {Conference} on {Computer} {Research} and {Development}},
	author = {Shi, Z. and Chen, L. and Chen, T.-E.},
	year = {2011},
	pages = {488--491}
}


@inproceedings{putra2012,
	title = {Industrial extreme programming practice's implementation in rational unified process on agile development theme},
	booktitle = {2012 {International} {Conference} on {Advanced} {Computer} {Science} and {Information} {Systems}, {ICACSIS} 2012 - {Proceedings}},
	author = {Putra, I.P.E.S. and Yuliawati, A. and Mursanto, P.},
	year = {2012},
	pages = {137--142}
}

@inproceedings{uikey2012,
	title = {An empirical study to design an effective agile project management framework},
	booktitle = {{ACM} {International} {Conference} {Proceeding} {Series}},
	author = {Uikey, N. and Suman, U.},
	year = {2012},
	pages = {385--390}
}

@article{poppendieck2012,
	title = {Lean software development: a tutorial},
	volume = {29},
	number = {5},
	journal = {IEEE Software},
	author = {Poppendieck, M. and Cusumano, M.A.},
	year = {2012},
	pages = {26--32}
}

@article{sletholt2012,
	title = {What do we know about scientific software development's agile practices?},
	volume = {14},
	number = {2},
	journal = {Computing in Science and Engineering},
	author = {Sletholt, M.T. and Hannay, J.E. and Pfahl, D. and Langtangen, H.P.},
	year = {2012},
	pages = {24--36}
}

@inproceedings{dyck2012,
	title = {Identifying common characteristics in fundamental, integrated, and agile software development methodologies},
	booktitle = {Proceedings of the {Annual} {Hawaii} {International} {Conference} on {System} {Sciences}},
	author = {Dyck, S. and Majchrzak, T.A.},
	year = {2012},
	pages = {5299--5308}
}

@inproceedings{eloranta2013,
	title = {Scrum anti-patterns - a empirical study},
	volume = {1},
	booktitle = {Proceedings - {Asia}-{Pacific} {Software} {Engineering} {Conference}, {APSEC}},
	author = {Eloranta, V.-P. and Koskimies, K. and Mikkonen, T. and Vuorinen, J.},
	year = {2013},
	pages = {503--510}
}

@inproceedings{kompella2014,
	title = {Agile methods, organizational culture and agility: some insights},
	booktitle = {8th {International} {Workshop} on {Cooperative} and {Human} {Aspects} of {Software} {Engineering}, {CHASE} 2014 - {Proceedings}},
	author = {Kompella, L.},
	year = {2014},
	pages = {40--47}
}

@book{meyer2014,
	series = {Agile!: the good, the hype and the ugly},
	title = {Agile!: the good, the hype and the ugly},
	volume = {9783319051550},
	author = {Meyer, B.},
	year = {2014},
	publisher = {Spring},
	address = { Cham }
}

@inproceedings{diebold2014,
	title = {Agile practices in practice - a mapping study},
	booktitle = {{ACM} {International} {Conference} {Proceeding} {Series}},
	author = {Diebold, P. and Dahlem, M.},
	year = {2014},
}

@article{papatheocharous2014,
	title = {Empirical evidence and state of practice of software agile teams},
	volume = {26},
	number = {9},
	journal = {Journal of Software: Evolution and Process},
	author = {Papatheocharous, E. and Andreou, A.S.},
	year = {2014},
	pages = {855--866}
}

@article{vijay2015,
	title = {Issues in scrum agile development principles and practices in software development},
	volume = {8},
	number = {35},
	journal = {Indian Journal of Science and Technology},
	author = {Vijay Anand, R. and Dinakaran, M.},
	year = {2015},
}

@inproceedings{agrawalla2015,
	title = {Towards a theoretical foundation for agile development},
	booktitle = {1st {IEEE} {International} {Symposium} on {Systems} {Engineering}, {ISSE} 2015 - {Proceedings}},
	author = {Agrawalla, R.K.},
	year = {2015},
	pages = {461--468}
}

@article{ghani2015,
	title = {Agile adoption in {IT} organizations},
	volume = {9},
	number = {8},
	journal = {KSII Transactions on Internet and Information Systems},
	author = {Ghani, I. and Bello, M.},
	year = {2015},
	pages = {3231--3248}
}

@book{gregory2015,
 	title = {Agile challenges in practice: a thematic analysis},
 	volume = {212},
 	author = {Gregory, P. and Barroca, L. and Taylor, K. and Salah, D. and Sharp, H.},
 	year = {2015},
}

@article{gregory2016-agile-challenges,
	title = "The challenges that challenge: Engaging with agile practitioners’ concerns",
	journal = "Information and Software Technology",
	volume = "77",
	pages = "92 - 104",
	year = "2016",
	issn = "0950-5849",
	doi = "https://doi.org/10.1016/j.infsof.2016.04.006",
	url = "http://www.sciencedirect.com/science/article/pii/S0950584916300623",
	author = "Peggy Gregory and Leonor Barroca and Helen Sharp and Advait Deshpande and Katie Taylor",
}

@article{dikert2016,
	title = {Challenges and success factors for large-scale agile transformations: a systematic literature review},
	volume = {119},
	journal = {Journal of Systems and Software},
	author = {Dikert, K. and Paasivaara, M. and Lassenius, C.},
	year = {2016},
	pages = {87--108}
}



@inproceedings{anwar2016,
	title = {Agile adoption case study, pains, challenges \& benefits},
	volume = {28-29-May-2016},
	booktitle = {{ACM} {International} {Conference} {Proceeding} {Series}},
	author = {Anwar, A. and Kamel, A.A. and Ahmed, E.},
	year = {2016},
	pages = {60--65}
}

@inproceedings{paasivaara2016,
	title = {Challenges and success factors for large-scale agile transformations - a research proposal and a pilot study},
	volume = {24-May-2016},
	booktitle = {{ACM} {International} {Conference} {Proceeding} {Series}},
	author = {Paasivaara, M. and Lassenius, C.},
	year = {2016},
}

@article{uikey2016,
	title = {Tailoring for agile methodologies: a framework for sustaining quality and productivity},
	volume = {23},
	number = {4},
	journal = {International Journal of Business Information Systems},
	author = {Uikey, N. and Suman, U.},
	year = {2016},
	pages = {432--455}
}

@article{nuottila2016,
	title = {Challenges of adopting agile methods in a public organization},
	volume = {4},
	number = {3},
	journal = {International Journal of Information Systems and Project Management},
	author = {Nuottila, J. and Aaltonen, K. and Kujala, J.},
	year = {2016},
	pages = {65--85}
}

@InProceedings{kropp2016,
	author="Kropp, Martin and Meier, Andreas and Biddle, Robert",
	editor="Abrahamsson, Pekka and Jedlitschka, Andreas and Nguyen Duc, Anh and Felderer, Michael and Amasaki, Sousuke and Mikkonen, Tommi",
	title="Agile Practices, Collaboration and Experience",
	booktitle="Product-Focused Software Process Improvement",
	year="2016",
	publisher="Springer International Publishing",
	address="Cham",
	pages="416--431",
	isbn="978-3-319-49094-6"
}

@article{jain2016,
	title = {Effectiveness of agile practices in global software development},
	volume = {9},
	number = {10},
	journal = {International Journal of Grid and Distributed Computing},
	author = {Jain, R. and Suman, U.},
	year = {2016},
	pages = {231--248}
}

@inproceedings{hoda2017,
	title = {Becoming agile: a grounded theory of agile transitions in practice},
	booktitle = {Proceedings - 2017 {IEEE}/{ACM} 39th {International} {Conference} on {Software} {Engineering}, {ICSE} 2017},
	author = {Hoda, R. and Noble, J.},
	year = {2017},
	pages = {141--151}
}

@inproceedings{silva2017,
	title = {Critical factors in agile software projects according to people, process and technology perspective},
	booktitle = {Proceedings - 6th {Brazilian} {Workshop} on {Agile} {Methods}, {WBMA} 2015},
	author = {Silva, K.M.B.D. and Santos, S.C.D.},
	year = {2017},
	pages = {48--54}
}

@inproceedings{sunner2017,
	title = {Agile: adapting to need of the hour: understanding agile methodology and agile techniques},
	booktitle = {Proceedings of the 2016 2nd {International} {Conference} on {Applied} and {Theoretical} {Computing} and {Communication} {Technology}, {iCATccT} 2016},
	author = {Sunner, D.},
	year = {2017},
	pages = {130--135}
}

@inproceedings{lacerda2018,
	title = {Factors that help in the implantation of agile methods: a systematic mapping of the liteature},
	volume = {2018-June},
	booktitle = {Iberian {Conference} on {Information} {Systems} and {Technologies}, {CISTI}},
	author = {Lacerda, L.L. and Furtado, F.},
	year = {2018},
	pages = {1--6}
}

@article{vallon2018,
	title = {Systematic literature review on agile practices in global software development},
	volume = {96},
	journal = {Information and Software Technology},
	author = {Vallon, R. and da Silva Estácio, B.J. and Prikladnicki, R. and Grechenig, T.},
	year = {2018},
	pages = {161--180}
}

@article{arora2017github,
  title={Supporting collaborative software development over GitHub},
  author={Arora, Ritu and Goel, Sanjay and Mittal, Ravi Kant},
  journal={Software: Practice and Experience},
  volume={47},
  number={10},
  pages={1393--1416},
  year={2017},
  publisher={Wiley Online Library}
}

@misc{neath2011githubissues20,
	title = {{Issues 2.0: The Next Generation}},
	author = {Kyle Neath},
	year = {2011},
	month = {Apr},
    howpublished = {https://github.blog/2011-04-09-issues-2-0-the-next-generation/},
    note = {Accessed: 2020-08-25},
}

@misc{warner2018github100millionrepo,
	title = {{Thank you for 100 million repositories}},
	author = {Jason Warner},
	year = {2018},
	month = {Nov},
    howpublished = {https://github.blog/2018-11-08-100m-repos/#:~:text=Today%20we%20reached%20a%20major,collaborating%20across%201.1%20billion%20contributions.},
    note = {Accessed: 2020-08-25},
}

@manual {racasan2020,
    title   = {How To Use GitHub for Agile Project Management},
    author  = {Mariana Racasan},
    year    = {2020},
    month   = {May},
    url     = {https://blog.zenhub.com/how-to-use-github-agile-project-management/}
}

@book{butler2016-zenhubBook, 
    title={Better Software \& Stronger Teams - Project Management for GitHub}, 
    publisher={ZenHub}, 
    author={Butler, Matt and Paquette, Paige}, 
    year={2016}
}

@article{jacksi2015-ejournaldesign,
  title={Design and implementation of online submission and peer review system: A case study of ejournal of university of zakho},
  author={Jacksi, Karwan},
  journal={International Journal of Scientific and Technology Researches},
  volume={4},
  number={8},
  pages={83--85},
  year={2015}
}

@article{steenweg2012,
  title={Software engineering process metamodels--a literature review},
  author={Steenweg, Ragna and Kuhrmann, Marco and M{\'e}ndez Fern{\'a}ndez, Daniel},
  journal={Technische Universit{\"a}t M{\"u}nchen, Tech. Rep. TUM-I1220},
  year={2012}
}

@book{mikowski2013SPA,
  title={Single page web applications: JavaScript end-to-end},
  author={Mikowski, Michael and Powell, Josh},
  year={2013},
  publisher={Manning Publications Co.}
}

@inproceedings{sadi2009apm3,
  title={{APM3: A Methodology Metamodel for Agile Project Management.}},
  author={Sadi, Mahsa Hasani and Ramsin, Raman},
  booktitle={SoMeT},
  pages={367--378},
  year={2009}
}

@inproceedings{ayed2012,
  title={A metamodel-based approach for customizing and assessing agile methods},
  author={Ayed, Hajer and Vanderose, Beno{\^\i}t and Habra, Naji},
  booktitle={Quality of Information and Communications Technology (QUATIC), 2012 Eighth International Conference on the},
  pages={66--74},
  year={2012},
  organization={IEEE}
}

@incollection{engels2010:metame,
  title={{A Meta-Method for Defining Software Engineering Methods}},
  author={Engels, Gregor and Sauer, Stefan},
  booktitle={Graph transformations and model-driven engineering},
  pages={411--440},
  year={2010},
  publisher={Springer}
}

@phdthesis{ternite2010:vmodellxt,
  author       = {Thomas Ternite}, 
  title        = {Variability of Development Models},
  school       = {Clausthal University of Technology},
  year         = 2010
}

@article{collierB1996-postmortem,
author = {Collier, B and DeMarco, T and Fearey, P},
issn = {0740-7459},
journal = {IEEE Software},
number = {4},
pages = {65-72},
publisher = {IEEE},
title = {A defined process for project post mortem review},
volume = {13},
year = {1996},
}


@book{goncalves-linders2015agile-retrospectives,
  title={Getting value out of agile retrospectives: a toolbox of retrospective exercises},
  author={Gon{\c{c}}alves, Luis and Linders, Ben},
  year={2015},
  publisher={Ben Linders Publishing}
}


@inproceedings{Ghaleb2020-bug-injection,
    author = {Ghaleb, Asem and Pattabiraman, Karthik},
    title = {How Effective Are Smart Contract Analysis Tools? Evaluating Smart Contract Static Analysis Tools Using Bug Injection},
    year = {2020},
    isbn = {9781450380089},
    publisher = {Association for Computing Machinery},
    address = {New York, NY, USA},
    url = {https://doi.org/10.1145/3395363.3397385},
    doi = {10.1145/3395363.3397385},
    booktitle = {Proceedings of the 29th ACM SIGSOFT International Symposium on Software Testing and Analysis},
    pages = {415–427},
    numpages = {13},
    location = {Virtual Event, USA},
    series = {ISSTA 2020}
}

@inproceedings{bonett2018-bug-injection,
  title={Discovering Flaws in Security-Focused Static Analysis Tools for Android using Systematic Mutation},
  author={R. Bonett and Kaushal Kafle and K. Moran and Adwait Nadkarni and D. Poshyvanyk},
  booktitle={USENIX Security Symposium},
  year={2018}
}

@article{dolan-gavitt2016-bug-injection,
  title={LAVA: Large-Scale Automated Vulnerability Addition},
  author={Brendan Dolan-Gavitt and P. Hulin and E. Kirda and T. Leek and A. Mambretti and William K. Robertson and F. Ulrich and R. Whelan},
  journal={2016 IEEE Symposium on Security and Privacy (SP)},
  year={2016},
  pages={110-121}
}

@article{pewny2016-bug-injection,
  title={EvilCoder: automated bug insertion},
  author={Jannik Pewny and Thorsten Holz},
  journal={Proceedings of the 32nd Annual Conference on Computer Security Applications},
  year={2016}
}

@article{eloranta2015-scrumbut,
    author = {Eloranta, Veli-Pekka and Koskimies, Kai and Mikkonen, Tommi},
    year = {2015},
    month = {12},
    pages = {},
    title = {Exploring {ScrumBut} – An Empirical Study of Scrum Anti-Patterns},
    volume = {74},
    journal = {Information and Software Technology},
    doi = {10.1016/j.infsof.2015.12.003}
}

@article{hassan2011-agile-adoption,
    author = {Hajjdiab, Hassan and Taleb, Al},
    year = {2011},
    month = {09},
    pages = {1-10},
    title = {Adopting Agile Software Development: Issues and Challenges},
    volume = {2},
    journal = {International Journal of Managing Value and Supply Chains},
    doi = {10.5121/ijmvsc.2011.2301}
}


@article{bermejo2014-agile-problems,
    author = {De Souza Bermejo, Paulo and Zambalde, Andre and Tonelli, Adriano and Souza, Samara and Zuppo, Larissa and Rosa, Priscila},
    year = {2014},
    month = {12},
    pages = {718-727},
    title = {Agile Principles and Achievement of Success in Software Development: A Quantitative Study in Brazilian Organizations},
    volume = {16},
    journal = {Procedia Technology},
    doi = {10.1016/j.protcy.2014.10.021}
}


@article{tarwani2016agile-agile-benefits,
  title={Agile methodologies in software maintenance: A systematic review},
  author={Tarwani, Sandhya and Chug, Anuradha},
  journal={Informatica},
  volume={40},
  number={4},
  year={2016}
}


@inproceedings{lopez2016problems,
  title={Problems in the adoption of agile-scrum methodologies: A systematic literature review},
  author={L{\'o}pez-Mart{\'\i}nez, Janeth and Ju{\'a}rez-Ram{\'\i}rez, Reyes and Huertas, Carlos and Jim{\'e}nez, Samantha and Guerra-Garc{\'\i}a, Cesar},
  booktitle={2016 4th international conference in software engineering research and innovation (conisoft)},
  pages={141--148},
  year={2016},
  organization={IEEE}
}

@inproceedings{mockus2000oss,
  title={A case study of open source software development: the Apache server},
  author={Mockus, Audris and Fielding, Roy T and Herbsleb, James},
  booktitle={Proceedings of the 22nd international conference on Software engineering},
  pages={263--272},
  year={2000}
}

@article{barlow2011-agile-adoption,
  title={Overview and guidance on agile development in large organizations},
  author={Barlow, Jordan B and Giboney, Justin and Keith, Mark J and Wilson, David and Schuetzler, Ryan M and Lowry, Paul Benjamin and Vance, Anthony},
  journal={Communications of the Association for Information Systems},
  volume={29},
  number={2},
  pages={25--44},
  year={2011}
}

@article{sidky2007-agile-adoption,
  title={A disciplined approach to adopting agile practices: the agile adoption framework},
  author={Sidky, Ahmed and Arthur, James and Bohner, Shawn},
  journal={Innovations in systems and software engineering},
  volume={3},
  number={3},
  pages={203--216},
  year={2007},
  publisher={Springer}
}

@article{gandomani2015-agile-adoption,
  title={An empirically-developed framework for Agile transition and adoption: A Grounded Theory approach},
  author={Gandomani, Taghi Javdani and Nafchi, Mina Ziaei},
  journal={Journal of Systems and Software},
  volume={107},
  pages={204--219},
  year={2015},
  publisher={Elsevier}
}


@phdthesis{esfahani2012-agile-adoption,
  title={Transitioning to agile: A framework for pre-adoption analysis using empirical knowledge and strategic modeling},
  author={Esfahani, Hesam Chiniforooshan},
  year={2012}
}

@inproceedings{rohunen2010-agile-adoption,
  title={Approaches to agile adoption in large settings: a comparison of the results from a literature analysis and an industrial inventory},
  author={Rohunen, Anna and Rodriguez, Pilar and Kuvaja, Pasi and Krzanik, Lech and Markkula, Jouni},
  booktitle={International Conference on Product Focused Software Process Improvement},
  pages={77--91},
  year={2010},
  organization={Springer}
}

@book{elssamadisy2008-agile-adoption-patterns,
  title={Agile Adoption Patterns: A Roadmap to Organizational Success (Adobe ebook)},
  author={Elssamadisy, Amr},
  year={2008},
  publisher={Addison-Wesley Professional}
}

@article{schweigert2014-agility-maturity-models-analysis,
  title={Agile maturity model: analysing agile maturity characteristics from the SPICE perspective},
  author={Schweigert, Tomas and Vohwinkel, Detlef and Korsaa, Morten and Nevalainen, Risto and Biro, Miklos},
  journal={Journal of Software: Evolution and Process},
  volume={26},
  number={5},
  pages={513--520},
  year={2014},
  publisher={Wiley Online Library}
}


@inproceedings{ozden2016-agility-assessment-tools-evaluation,
  title={Evaluation of agility assessment tools: a multiple case study},
  author={Adal{\i}, Onat Ege and {\"O}zcan-Top, {\"O}zden and Demir{\"o}rs, Onur},
  booktitle={International Conference on Software Process Improvement and Capability Determination},
  pages={135--149},
  year={2016},
  organization={Springer}
}


@inproceedings{ullah2013-automated-compliance-tool,
  author={K. W. {Ullah} and A. S. {Ahmed} and J. {Ylitalo}},
  booktitle={2013 12th IEEE International Conference on Trust, Security and Privacy in Computing and Communications}, 
  title={Towards Building an Automated Security Compliance Tool for the Cloud}, 
  year={2013},
  volume={},
  number={},
  pages={1587-1593},
}

@inproceedings{dimyadi2017-automating-compliance,
	author="Dimyadi, Johannes and Amor, Robert",
	title="Automating Conventional Compliance Audit Processes",
	booktitle="Product Lifecycle Management and the Industry of the Future",
	year="2017",
	publisher="Springer International Publishing",
	address="Cham",
	pages="324--334",
}

@inproceedings{park2012-real-time-auditing,
  author={J. S. {Park} and E. {Spetka} and H. {Rasheed} and P. {Ratazzi} and K. J. {Han}},
  booktitle={2012 26th International Conference on Advanced Information Networking and Applications Workshops}, 
  title={Near-Real-Time Cloud Auditing for Rapid Response}, 
  year={2012},
  volume={},
  number={},
  pages={1252-1257},
}

@inproceedings{moha2006,
  author={N. {Moha} and Y. {Gueheneuc} and P. {Leduc}},
  booktitle={21st IEEE/ACM International Conference on Automated Software Engineering (ASE'06)}, 
  title={Automatic Generation of Detection Algorithms for Design Defects}, 
  year={2006},
  volume={},
  number={},
  pages={297-300},
}

@article{kharbili2008-passive-active-approach,
	author = {Kharbili, M. and Sebastian, Stein and Markovic, I. and Pulvermüller, E.},
	year = {2008},
	month = {01},
	pages = {1-15},
	title = {{Towards a Framework for Semantic Business Process Compliance Management}},
	volume = {339},
	journal = {CEUR Workshop Proceedings}
}


@inproceedings{thullner2011-proactive-compliance-monitoring,
  author={R. {Thullner} and S. {Rozsnyai} and J. {Schiefer} and H. {Obweger} and M. {Suntinger}},
  booktitle={2011 IEEE 15th International Enterprise Distributed Object Computing Conference Workshops}, 
  title={Proactive Business Process Compliance Monitoring with Event-Based Systems}, 
  year={2011},
  volume={},
  number={},
  pages={429-437},
}

@inproceedings{mulo2009-monitoring-event,
  title={Monitoring web service event trails for business compliance},
  author={Mulo, Emmanuel and Zdun, Uwe and Dustdar, Schahram},
  booktitle={2009 IEEE International Conference on Service-Oriented Computing and Applications (SOCA)},
  pages={1--8},
  year={2009},
  organization={IEEE}
}


@article{turetken2012-capture-compliance-requirements,
  author={O. {Turetken} and A. {Elgammal} and W. {van den Heuvel} and M. P. {Papazoglou}},
  journal={IEEE Software}, 
  title={Capturing Compliance Requirements: A Pattern-Based Approach}, 
  year={2012},
  volume={29},
  number={3},
  pages={28-36},
}


@inproceedings{vassiliadis2002etl,
  title={Conceptual modeling for ETL processes},
  author={Vassiliadis, Panos and Simitsis, Alkis and Skiadopoulos, Spiros},
  booktitle={Proceedings of the 5th ACM international workshop on Data Warehousing and OLAP},
  pages={14--21},
  year={2002}
}

@article{sajad2016-spm,
  title={Software Project Management: Tools assessment, Comparison and suggestions for future development},
  author={Sajad, Muhammad and Sadiq, Muhammad and Naveed, Khawar and Iqbal, Muhammad Shahid},
  journal={International Journal of Computer Science and Network Security (IJCSNS)},
  volume={16},
  number={1},
  pages={31},
  year={2016},
  publisher={International Journal of Computer Science and Network Security}
}


@inproceedings{bleiel2016-collaborating-github,
  title={Collaborating in GitHub},
  author={Bleiel, Nicky},
  booktitle={2016 IEEE International Professional Communication Conference (IPCC)},
  pages={1--3},
  year={2016},
  organization={IEEE}
}


@manual{stormconsulting2008-agile-enterprise-survey,
      title  = "Agile Enterprise Survey",
      author = "Storm-Consulting",
      url    = "http://www.storm-consulting.com/agile-enterprise-survey/",
      year   = "2008"
}


@manual { lagestee2012-agile-health-dashboard,
    title   = "Agile Health Dashboard",
    author  = "Len Lagestee",
    year    = "2012",
    url     = "http://illustratedagile.com/2012/09/25/how-to-measure-team-agility/"
}


@manual { krebs2011-agile-journey-index,
    title   = {Agile Journey Index},
    author  = {Bill Krebs},
    year    = {2011},
    url     = {http://www.agiledimensions.com/blog/}
}


@manual {infotech2013-agile-process-assessment-tool,
    author  = {Infotech},
    title   = {Agile Process Assessment Tool},
    year    = {2013},
    url     = {https://www.infotech.com/research/it-agile-process-assessment-tool}
}

@manual { britsch2017-agility-questionnaire,
    author  = {Marcel Britsch},
    title   = {{Agility Questionnaire}},
    year    = {2017},
    url     = {https://thedigitalbusinessanalyst.co.uk/agility-questionnaire-130b03133b98}

}

@manual {cohn2015-comparative-agile,
    title   = {Comparative Agile},
    author  = {Mike Cohn and Ken Rubin},
    year    = {2015},
    url     = {https://www.comparativeagility.com/capabilities/agile-assessment},
}

@manual {achouiantz2013-depth-of-kanban,
    title   = {{Depth of Kanban}},
    author  = {Christophe Achouiantz},
    year    = {2013},
    url     = {http://leanagileprojects.blogspot.com/2013/03/depth-of-kanban-good-coaching-tool.html}
}

@book{anderson2010kanban,
  title={Kanban: successful evolutionary change for your technology business},
  author={Anderson, David J},
  year={2010},
  publisher={Blue Hole Press}
}

@manual {eliassengroup2013-enterprise-agility-maturity-matrix,
    title   = {{Enterprise Agility Maturity Matrix}},
    author  = {Eliassen-Group},
    year    = {2013},
    url     = {http://blog.eliassen.com/introducing-the-enterprise-agility-maturity-matrix},
}

@manual {ibm2014-ibm-devops-practices-self-assessment,
    title   = {{IBM DevOps Practices Self-Assessment}},
    author  = {IBM},
    year    = {2014 (accessed October 1, 2020)},
    url     = {http://www.surveygizmo.com/s3/1659087/IBM-DevOps-Self-Assessment},
}

@inproceedings{sureshchandra2008-agile-adoption,
  title={Adopting agile in distributed development},
  author={Sureshchandra, Kalpana and Shrinivasavadhani, Jagadish},
  booktitle={2008 IEEE International Conference on Global Software Engineering},
  pages={217--221},
  year={2008},
  organization={IEEE}
}

@inproceedings{packlick2007agile,
  title={The agile maturity map a goal oriented approach to agile improvement},
  author={Packlick, Jay},
  booktitle={Agile 2007 (AGILE 2007)},
  pages={266--271},
  year={2007},
  organization={IEEE}
}

@article{patel2009-amm,
  title={Agile maturity model (AMM): a software process improvement framework for agile software development practices},
  author={Patel, Chetankumar and Ramachandran, Muthu},
  journal={International Journal of Software Engineering, IJSE},
  volume={2},
  number={1},
  pages={3--28},
  year={2009}
}


@article{ambler2009-asm,
  title={The agile scaling model (ASM): adapting agile methods for complex environments},
  author={Ambler, Scott W},
  journal={Environments},
  pages={1--35},
  year={2009}
}

@manual {pettit2006-innovation-maturity-model,
    title   = {Innovation Maturity Model},
    author  = {Ross Pettit},
    year    = {2006 },
    url     = {http://www.rosspettit.com/2007/02/innovation-maturity-model.html}
}

@article{turetken2017assessing,
  title={Assessing the adoption level of scaled agile development: a maturity model for Scaled Agile Framework},
  author={Turetken, Oktay and Stojanov, Igor and Trienekens, Jos JM},
  journal={Journal of Software: Evolution and process},
  volume={29},
  number={6},
  pages={e1796},
  year={2017},
  publisher={Wiley Online Library}
}

@inproceedings{nawrocki2001toward-maturity-model-xp,
  title={Toward maturity model for extreme programming},
  author={Nawrocki, Jerzy and Walter, Bartosz and Wojciechowski, Adam},
  booktitle={Proceedings 27th EUROMICRO Conference. 2001: A Net Odyssey},
  pages={233--239},
  year={2001},
  organization={IEEE}
}

@manual {openapi,
    title   = {OpenAPI Specification},
    author  = {The Linux Foundation},
    year    = {2018},
    url     = {https://www.openapis.org/}
}

@inproceedings{koren2018-openapi,
author = {Koren, Istv\'{a}n and Klamma, Ralf},
title = {The Exploitation of OpenAPI Documentation for the Generation of Web Frontends},
year = {2018},
isbn = {9781450356404},
publisher = {International World Wide Web Conferences Steering Committee},
address = {Republic and Canton of Geneva, CHE},
url = {https://doi.org/10.1145/3184558.3188740},
doi = {10.1145/3184558.3188740},
booktitle = {Companion Proceedings of the The Web Conference 2018},
pages = {781–787},
numpages = {7},
keywords = {interaction design, web components, ifml, openapi},
location = {Lyon, France},
series = {WWW '18}
}


@inproceedings{fontana2013codesmell,
  title={Code smell detection: Towards a machine learning-based approach},
  author={Fontana, Francesca Arcelli and Zanoni, Marco and Marino, Alessandro and M{\"a}ntyl{\"a}, Mika V},
  booktitle={2013 IEEE International Conference on Software Maintenance},
  pages={396--399},
  year={2013},
  organization={IEEE}
}

@article{paiva2017evaluationcodesmells,
  title={On the evaluation of code smells and detection tools},
  author={Paiva, Thanis and Damasceno, Amanda and Figueiredo, Eduardo and Sant’Anna, Cl{\'a}udio},
  journal={Journal of Software Engineering Research and Development},
  volume={5},
  number={1},
  pages={7},
  year={2017},
  publisher={Springer}
}

@inproceedings{fernandes2016-evaluationcodesmells,
author = {Fernandes, Eduardo and Oliveira, Johnatan and Vale, Gustavo and Paiva, Thanis and Figueiredo, Eduardo},
title = {A Review-Based Comparative Study of Bad Smell Detection Tools},
year = {2016},
isbn = {9781450336918},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2915970.2915984},
doi = {10.1145/2915970.2915984},
booktitle = {Proceedings of the 20th International Conference on Evaluation and Assessment in Software Engineering},
articleno = {18},
numpages = {12},
keywords = {comparative study, bad smells, detection tools, systematic literature review},
location = {Limerick, Ireland},
series = {EASE '16}
}


@manual {nowinski2016-agileassessment,
    title = {Agile Assessment},
    author = {Piotr Nowinski},
    year = {2016},
    url = {http://piotr-nowinski.pl/agile-assessment/}
}

@manual {seuffert2019-KarlskronaTestOnline,
    title = {Karlskrona test online},
    author = {Mark Seuffert},
    year = {2019},
    url = {https://mayberg.se/karlskrona-test-online}
}


@manual {gunnerson2015-agileteamevaluation,
    title = {{Agile Team Evaluation}},
    author = {Eric Gunnerson},
    year = {2015},
    url = {https://docs.microsoft.com/en-us/archive/blogs/ericgu/agile-team-evaluation}
}

@manual{wolpers2016-cargocultagilechecklist,
    title = {Cargo Cult Agile Checklist},
    author = {Stefan Wolpers},
    year = {2016},
    url ={https://age-of-product.com/cargo-cult-agile-state-agile-checklist-organization/}
}

@manual{scaledagile-metrics,
    title = {Metrics - Scaled Agile Framework},
    author = {Scaled Agile},
    url = {https://www.scaledagileframework.com/metrics/},
    year = {2012}
}

@manual{scaledagile-organizationalAgilitySelfAssessment,
    title = {Organizational Agility Self-Assessment},
    author = {Scaled Agile},
    url = {https://www.scaledagileframework.com/metrics/#PF9},
    year = {2012}
}

@manual{scaledagile-organizationalAgility,
    title = {Organizational Agility},
    author = {Scaled Agile},
    url = {https://www.scaledagileframework.com/organizational-agility/},
    year = {2012}
}


@manual{scaledagile-teamAndTechnicalAgilitySelfAssessment,
    title = {Team and Technical Agility Self-Assessment},
    author = {Scaled Agile},
    url = {https://www.scaledagileframework.com/metrics/#T4},
    year = {2012}
}

@manual{scaledagile-teamAndTechnicalAgility,
    title = {Team and Technical Agility},
    author = {Scaled Agile},
    url = {https://www.scaledagileframework.com/team-and-technical-agility/},
    year = {2012}
}

@manual{james2007-scrummasterChecklist,
    title = {ScrumMaster Checklist},
    author = {Michael James},
    year = {2007},
    url = {https://scrummasterchecklist.org/pdf/ScrumMaster_Checklist_12_unbranded.pdf}
}

@manual{janlen2014-Barometer,
    title = {Team Barometer},
    author = {Jimmy Janlén},
    year = {2014},
    url = {https://blog.crisp.se/2014/01/30/jimmyjanlen/team-barometer-self-evaluation-tool}
}

@manual{lewis2016-stormAgileEnterpriseSurvey,
    title = {Agile Enterprise Survey},
    author = {Russ Lewis and Roy Wendler},
    year = {2016},
    url = {http://www.storm-consulting.com/agile-enterprise-survey/}
}

@article{erande2008CAMT,
  title={Measuring agility of organizations-a comprehensive agility measurement tool (CAMT)},
  author={Erande, Ameya S and Verma, Alok K},
  journal={International journal of applied management and technology},
  volume={6},
  number={3},
  year={2008}
}


@article{cmmi2000,
  title={{CMMI for Systems Engineering/Software Engineering/Integrated Product and Process Development/Supplier Sourcing, Version 1.02}},
  author={Team, CMMI Product},
  journal={CMU/SEI},
  year={2000}
}

@techreport{ISO-IEC-15504,
	type = {Standard},
	key = {ISO/IEC 15504},
	year = {2002},
	title = {{ISO/IEC 15504: Information Technology - Process Assessment, Part 1 to Part 5}},
	volume = {2014},
	address = {Geneva, CH},
	institution = {International Organization for Standardization}
}

@inproceedings{lui2005roadmap-xp,
  title={{A Road Map for Implementing eXtreme Programming}},
  author={Lui, Kim Man and Chan, Keith CC},
  booktitle={Software Process Workshop},
  pages={474--481},
  year={2005},
  organization={Springer}
}


@manual {linders-list-agile-assessments,
    title = {Agile self-assessments},
    author = {Ben Linders},
    url = {https://www.benlinders.com/tools/agile-self-assessments/},
    year = {2014}
}


@manual{lebow2018-versionOneAgileAssessment, 
    title = {{Agile Assessment: Test Your Team's Agility}},
    author = {Jodi Lebow},
    url = {https://digital.ai/resources/agile-101/agile-assessment},
    year = {2018}
}

@manual{little2012-JoesUnofficialScrumChecklist,
    title = {{Joe's	Unofficial Scrum Checklist}},
    author = {Joseph H. Little},
    url = {http://agileconsortium.pbworks.com/w/file/fetch/66642311/Joe\%E2\%80\%99s\%20Unofficial\%20Scrum\%20CheckList\%20V13.pdf},
    year = {2012}

}


@book{linders2019-TheAgileSelf-AssessmentGame,
  title={The Agile Self-assessment Game},
  author={Ben Linders},
  url = {https://www.benlinders.com/game/},
  year={2019}
}

@manual{glover2012-ScrumChecklist2012,
    title = {Scrum Checklist 2012},
    author = {Boris Glover},
    url = {https://www.infoq.com/minibooks/scrum-checklists/},
    year = {2012}
}


@manual{vodde2010-NokiaTest,
    title = {Nokia Test},
    author = {Bas Vodde and Jeff Sutherland},
    url = {https://www.scruminc.com/official-scrumbutt-test-otherwise-known/},
    year = {2010}
}

@manual{hawks2013-ScrumAssessmentSeries,
    title = {Scrum Assessment Series},
    author = {David Hawks},
    year = {2013},
    url = {https://agilevelocity.com/scrum-assessment-series/}
}

@manual{scrumOrg2020-OpenAssessments,
    title = {Open Assessments},
    author = {Scrum.Org},
    year = {2020},
    url = {https://www.scrum.org/open-assessments}
}


@manual{kniberg2014-SquadHealthCheckModel,
    title = {Squad Health Check Model},
    author = {Henrik Kniberg and Kristian Lindwall},
    year = {2014},
    url = {https://engineering.atspotify.com/2014/09/16/squad-health-check-model/}
}


@manual{yeret2013LeanAgileDepthAssessmentChecklistA3,
    title = {Lean/Agile Depth Assessment Checklist A3},
    author = {Yuval Yeret},
    year = {2013},
    url = {https://www.slideshare.net/yyeret/leanagile-depth-assessment}
}

@manual{schuurkes2017-TestMaturityCardGame,
    title = {Test Maturity Card Game},
    author = {Huib Schoots and Joep Schuurkes},
    year = {2017},
    url = {https://www.huibschoots.nl/wordpress/wp-content/uploads/2017/02/Test-Improvement-Huib-Schoots-Joep-Schuurkes.pdf}
}

@manual{verwijs2017TeamMetrics,
    title = {TeamMetrics},
    author =  {Christiaan Verwijs},
    year = {2017},
    url = {https://teammetrics.theliberators.com/}
}

@manual{nielsen2011-FiveKeyNumbersToAssessYourAgileEngineeringPractices,
    title = {Five key numbers to gauge your agile engineering efforts},
    author = {Jeff Nielsen},
    year = {2011},
    url = {https://www.slideshare.net/jeffreymads/five-key-numbers-to-gauge-your-agile-engineering-efforts-7980346}
}

@manual{gao2020AgileAssessmentGuide,
    title = {Agile Assessment Guide},
    author = {U.S. Government Accountability Office GAO},
    year = {2020},
    url = {https://www.gao.gov/assets/710/709711.pdf}
}


@manual{hendrickson2008-Back-of-a-NapkinAgileAssessment,
    title = {Back-of-a-Napkin Agile Assessment},
    author = {Elisabeth Hendrickson},
    year = {2008},
    url = {https://testobsessed.com/2008/11/back-of-a-napkin-agile-assessment/}
}

@manual{spolsky2000-JoelTest,
    title = {The Joel Test: 12 Steps to Better Code},
    author = {Joel Spolsky},
    year = {2000},
    url = {https://www.joelonsoftware.com/2000/08/09/the-joel-test-12-steps-to-better-code/}
}

@manual{shoukath2012-AreYouReallyAgile,
    title = {Are you really agile?},
    author = {Nisha Shoukath},
    year = {2012},
    url = {https://blog.people10.com/are-you-really-agile-a-free-assessment-here/}
}

@manual{hogan2017-VisualManagementSelf-Assessment,
    title = {Visual Management Self-Assessment},
    author = {Ben Hogan},
    year = {2017},
    url = {http://agileben.com/blog/kanban-online-assessment}
}

@manual{mccalla2016-LeanAgileIntelligence,
    title = {Lean Agile Intelligence},
    author = {Michael McCalla and James Gifford},
    year = {2016},
    url = {https://www.leanagileintelligence.com/}
}

@manual{sfirlogea2017-Retropoly,
    title = {Retropoly},
    author = {Sorin Sfirlogea and Florian Georgescu},
    year = {2017},
    url ={https://www.agilepractice.eu/retropoly/}
}

@manual{sfirlogea2020-AgileExcellerate,
    title = {Agile Excellerate},
    author = {Sorin Sfirlogea and Florian Georgescu},
    year = {2020},
    url ={https://www.agilepractice.eu/agile-excellerate/}
}

@book{eoyang2001conditions,
  title={Conditions for self-organizing in human systems},
  author={Eoyang, Glenda Holladay},
  year={2001},
  publisher={Union Institute}
}



@inproceedings{lencioni2012five,
  title={The five dysfunctions of a team},
  author={Lencioni, Patrick},
  booktitle={A workshop for teams. Pfeiffer, a Wiley Imprint},
  year={2012}
}

@book{covey2006speed,
  title={The speed of trust: The one thing that changes everything},
  author={Covey, Stephen R and Merrill, Rebecca R},
  year={2006},
  publisher={Simon and schuster}
}

@manual{balbes2015-HowAgileAreYou,
    title = {{How Agile Are You? Let's Actually Measure It!}},
    author = {Mark Balbes},
    year = {2015},
    url = {https://adtmag.com/articles/2015/12/15/balbes-agile-model-0-intro.aspx}
}

@manual {parry2009QuickSelf-Assessment,
    title = {Quick self-assessment of your organization’s agility},
    author = {Charles Parry},
    year = {2009},
    url = {http://www.signetconsulting.com/action_items/assessment.php}
}


@manual{chiva2019-KanbanMaturityAssessment,
    title = {{Kanban Maturity Assessment}},
    author = {Gerard Chiva},
    year = {2019},
    url = {https://aktiasolutions.com/kanban-maturity-assessment/}
}

@manual{hoffmann2018-AgileAlert,
    title = {Agile Alert},
    author = {Rainer Hoffmann and Tilman Bona and Serge Petit},
    year = {2018},
    url = {https://huz.de/en/agile-alert/}
}

@manual{yodiz2017-TeamAgilitySelfAssessment,
    title = {Team Agility Self Assessment},
    author = {Yodiz},
    year = {2017},
    url = {https://www.yodiz.com/blog/how-agile-is-your-team-take-our-team-agility-self-assessment-to-find-out/}
}

@manual{burlton2018-BusinessAgilityManifesto,
    title = {Business Agility Manifesto},
    author = {Roger T. Burlton and Ronald G. Ross and John A. Zachman},
    year = {2018},
    url = {https://busagilitymanifesto.org/accompaniments/supplements/diagnostics}
}

@manual{ribeiro2018-EnterpriseBusinessAgilityMaturitySurvey,
    title = {Enterprise Business Agility Maturity Survey},
    author = {Eduardo Ribeiro},
    year = {2018},
    url = {https://beyondleanagile.com/2018/12/12/enterprise-business-agility-maturity-survey/}
}

@manual{albrecht2020-MeasureTeam,
    title = {Measure.team},
    author = {Kelly Albrecht and Sean Eddings},
    year = {2020},
    url = {https://measure.team/}

}

@manual{dod2018-DIBGuide,
    title = {DIB Guide: Detecting Agile BS},
    author = {{Department of Defense DOD}},
    year = {2018},
    url = {https://media.defense.gov/2018/Oct/09/2002049591/-1/-1/0/DIB_DETECTING_AGILE_BS_2018.10.05.PDF}
}

@manual{BPMI2019-AgileSkillsSelf-Assessment,
    title = {Agile Skills Self-Assessment},
    author = {BPM Institute BPMI},
    year = {2019},
    url = {https://www.bpminstitute.org/skills-self-assessments#}
}

@manual{bonamassa2018AgileAdoptionInterview,
    title = {Agile Adoption Interview},
    author = {Michael Bonamassa},
    year = {2018},
    url = {https://pladcloud.typeform.com/to/HjcVKG}
}

@manual{finite2019-A50PointTest,
    title = {{How Agile are you? A 50 Point Test}},
    author = {Finite},
    year = {2019},
    url = {https://www.finite.com.au/blog/2019/08/how-agile-are-you/}
}


@book{yin2003-casestudy-design,
  title={{Case Study Research: Design and methods}},
  author={Robert K Yin},
  volume={3},
  year={2003},
  publisher = {SAGE},
  edition = {5}
}

@article{runeson2009-casestudy-guidelines,
  title={Guidelines for conducting and reporting case study research in software engineering},
  author={Runeson, Per and H{\"o}st, Martin},
  journal={Empirical software engineering},
  volume={14},
  number={2},
  pages={131},
  year={2009},
  publisher={Springer}
}



@manual{sandoval2018-openapi,
    title = {What Should You Consider Before OpenAPI Adoption?},
    author = {Kristopher Sandoval},
    year = {2018},
    url = {https://nordicapis.com/what-should-you-consider-before-openapi-adoption/#:~:text=OpenAPI\%20Specification\%20can\%20be\%20used,and\%20visualize\%20RESTful\%20web\%20services.}
}


@phdthesis{renata2019phdthesis,
    title    = {Mapeamento entre Representações de Processo e Projeto de Software},
    school   = {UFRJ/ COPPE/ Programa de Engenharia de Sistemas e Computação},
    author   = {Santos, Renata Mesquita da Silva},
    year     = {2019},
}


@book{grossman2012information-retrieval,
  title={Information retrieval: Algorithms and heuristics},
  author={Grossman, David A and Frieder, Ophir},
  volume={15},
  year={2012},
  publisher={Springer Science \& Business Media}
}


@manual{pisuwala2019-agile-development-cycle,
    title = {A comprehensive guide on agile methods for modern software development},
    author = {Ubaid Pisuwala},
    year = {2019},
    url = {https://www.peerbits.com/blog/agile-software-development.html}
}


@article{larman2003-agile-brief-history,
  title={Iterative and incremental developments. a brief history},
  author={Larman, Craig and Basili, Victor R},
  journal={Computer},
  volume={36},
  number={6},
  pages={47--56},
  year={2003},
  publisher={IEEE}
}

@manual{takeuchi1996-scrum,
    title = {{The New New Product Development Game}},
    author = {Hirotaka Takeuchi and Ikujiro Nonaka},
    year = {1986},
    url = {https://hbr.org/1986/01/the-new-new-product-development-game}
}


@article{wu2017-likert-scales,
  title={Can Likert scales be treated as interval scales?—A Simulation study},
  author={Wu, Huiping and Leung, Shing-On},
  journal={Journal of Social Service Research},
  volume={43},
  number={4},
  pages={527--532},
  year={2017},
  publisher={Taylor \& Francis}
}

@article{hodge2007-likert-scales,
  title={Phrase completion scales: a better measurement approach than Likert scales?},
  author={Hodge, David R and Gillespie, David F},
  journal={Journal of Social Service Research},
  volume={33},
  number={4},
  pages={1--12},
  year={2007},
  publisher={Taylor \& Francis}
}

@article{carifio2008-likert-scales-resolving-50-year,
  title={Resolving the 50-year debate around using and misusing Likert scales},
  author={Carifio, James and Perla, Rocco},
  journal={Medical education},
  volume={42},
  number={12},
  pages={1150--1152},
  year={2008},
  publisher={Blackwell Publishing Ltd Oxford, UK}
}

@article{bishop2015-likert-scales-use,
  title={Use and misuse of the Likert item responses and other ordinal measures},
  author={Bishop, Phillip A and Herron, Robert L},
  journal={International journal of exercise science},
  volume={8},
  number={3},
  pages={297},
  year={2015},
  publisher={Western Kentucky University}
}


@article{joshi2015-likert-scale,
  title={Likert scale: Explored and explained},
  author={Joshi, Ankur and Kale, Saket and Chandel, Satish and Pal, D Kumar},
  journal={Current Journal of Applied Science and Technology},
  pages={396--403},
  year={2015}
}

@article{leung2011-likert-scale,
  title={A comparison of psychometric properties and normality in 4-, 5-, 6-, and 11-point Likert scales},
  author={Leung, Shing-On},
  journal={Journal of Social Service Research},
  volume={37},
  number={4},
  pages={412--421},
  year={2011},
  publisher={Taylor \& Francis}
}


@article{kuzon1996-seven-sins-Likert-scale,
  title={The seven deadly sins of statistical analysis},
  author={Kuzon, William and Urbanchek, Melanie and McCabe, Steven},
  journal={Annals of plastic surgery},
  volume={37},
  pages={265--272},
  year={1996}
}

@article{jamieson2004-likert,
  title={Likert scales: How to (ab) use them?},
  author={Jamieson, Susan},
  journal={Medical education},
  volume={38},
  number={12},
  pages={1217--1218},
  year={2004}
}

@article{stevens1946-likert,
  title={On the theory of scales of measurement},
  author={Stevens, Stanley Smith and others},
  year={1946},
  month = {Jun},
  volume = {103},
  pages={677--680},
  journal={Science, New Series},
  publisher={Bobbs-Merrill, College Division}
}


@article{knapp1990-likert,
  title={Treating ordinal scales as interval scales: an attempt to resolve the controversy},
  author={Knapp, Thomas R},
  journal={Nursing research},
  volume={39},
  number={2},
  pages={121--123},
  year={1990}
}


@article{borgatta1980-likert,
  title={Level of measurement: Once over again},
  author={Borgatta, Edgar F and Bohrnstedt, George W},
  journal={Sociological Methods \& Research},
  volume={9},
  number={2},
  pages={147--160},
  year={1980},
  publisher={Sage Publications Sage CA: Thousand Oaks, CA}
}
